Road Network Representation Learning: A Dual Graph based Approach

Road network is a critical infrastructure powering many applications including transportation, mobility and logistics in real life. To leverage the input of a road network across these different applications, it is necessary to learn the representations of the roads in the form of vectors, which is named \emph{road network representation learning} (RNRL). While several models have been proposed for RNRL, they capture the pairwise relationships/connections among roads only (i.e., as a simple graph), and fail to capture among roads the high-order relationships (e.g., those roads that jointly form a local region usually have similar features such as speed limit) and long-range relationships (e.g., some roads that are far apart may have similar semantics such as being roads in residential areas). Motivated by this, we propose to construct a \emph{hypergraph}, where each hyperedge corresponds to a set of multiple roads forming a region. The constructed hypergraph would naturally capture the high-order relationships among roads with hyperedges. We then allow information propagation via both the edges in the simple graph and the hyperedges in the hypergraph in a graph neural network context. The graph reconstruction and hypergraph reconstruction tasks are conventional ones and can capture structural information. The hyperedge classification task can capture long-range relationships between pairs of roads that belong to hyperedges with the same label. We call the resulting model \emph{HyperRoad}. We further extend HyperRoad to problem settings when additional inputs of road attributes and/or trajectories that are generated on the roads are available.

==> inputs/conclusion.tex <==
\section{Conclusion}
In this paper, we introduce a new structure named hypergraph into the road network representation learning problem. Based on that we propose a novel end-to-end pre-training framework HyperRoad, which features in the schemes of dual-channel aggregation mechanism to enhance model expressive power, and bi-level self-supervised pretext tasks (graph-level and hypergraph-level respectively) to capture both local and global road correlations. Extensive experiments on five downstream tasks demonstrate the great improvements of our model compared with existing baselines. The ablation and case study results also validate the necessity of introducing hypergraph modeling in road network settings.   

==> inputs/experiment_results.tex <==
\section{Experimental Results}
\label{sec:expresult}

In this section, we first conduct comprehensive comparison with the state-of-the-art road network representation learning methods in 5 downstream applications. To justify the module designs in HyperRoad and demonstrate the effectiveness, we then perform ablation studies in Section \ref{sec:q2}. Finally, we give discussions on parameter analysis and present a case study on \textit{Singapore} dataset to analyze what the learned road embeddings represent in Section \ref{sec:q3} and \ref{sec:q4}.

\begin{table*}[t!]
	\renewcommand{\arraystretch}{1.2} 
	\centering 
	\caption{Results for road segment based applications.}
    \normalsize
	\resizebox{1.0\linewidth}{!}{
		\begin{tabular}{c|ccc|ccc|ccc|ccc}
			\toprule
			\multirow{4}{*}{Method} & \multicolumn{6}{c|}{{\textbf{ One/Two Way}}} & \multicolumn{6}{c}{{\textbf{No. of Lanes}}}  \\
			\cmidrule{2-13}
			& \multicolumn{3}{c|}{{\it Singapore}} & \multicolumn{3}{c|}{{\it Xi'an}} & \multicolumn{3}{c|}{{\it Singapore}} & \multicolumn{3}{c}{{\it Xi'an}} \\
			\cmidrule{2-13}
			& Micro-F1 & Macro-F1 & Weighted-F1 & Micro-F1 & Macro-F1 & Weighted-F1 & Micro-F1 & Macro-F1 & Weighted-F1 & Micro-F1 & Macro-F1 & Weighted-F1  \\ \midrule
			DeepWalk & 0.7313 & 0.5027 & 0.6517 & 0.5888 & 0.5647 & 0.5758 & 0.4766 & 0.1082 & 0.3089 & 0.5498 & 0.2009 & 0.4209\\
			Node2Vec & 0.7213 & 0.4221 & 0.6059 & 0.5858 & 0.5638 & 0.5743 & 0.4773 & 0.1077 & 0.3087 & 0.5600 & 0.2675 & 0.4789\\
			LINE & \underline{0.7652} & 0.6018 & 0.7117 & 0.6032 & 0.5909 & 0.5985 & 0.4772 & 0.1094 & 0.3101 & 0.5504 & 0.1900 & 0.4070\\
			SDNE & 0.7199 & 0.4226 & 0.6058 & 0.5686 & 0.5114 & 0.5295 & 0.4778 & 0.1117 & 0.3120 & 0.5504 & 0.1833 & 0.3998\\
			\midrule
		    GAE & 0.7135 & 0.4935 & 0.6342 & \underline{0.6676} & \underline{0.6650} & \underline{0.6677} & 0.4790 & 0.1248 & 0.3186 & \underline{0.5827} & \underline{0.3383} & \underline{0.5235}\\
		    GraphSAGE & 0.7170 & 0.4829 & 0.6296 & 0.6452 & 0.6398 & 0.6438 & 0.4793 & 0.1228 & 0.3170 & 0.5794 & 0.2990 & 0.5181\\
		    \midrule
		    RFN & 0.7410 & 0.5995 & 0.6990 & 0.6305 & 0.6213 & 0.6267 & 0.4784 & 0.1177 & 0.3154 & 0.5596 & 0.2757 & 0.4737\\
		    IRN2Vec & 0.7085 & 0.4538 & 0.6110 & 0.6274 & 0.6100 & 0.6175 & \underline{0.4793} & \underline{0.1271} & \underline{0.3190} & 0.5677 & 0.2176 & 0.4508\\ 
		    HRNR & 0.7226 & \underline{0.6379} & \underline{0.7145} & 0.6659 & 0.6606 & 0.6652 & 0.4767 & 0.1076 & 0.3078 & 0.5601 & 0.2957 & 0.4547\\ 
		    \midrule
			HyperRoad & \textbf{0.7864} & \textbf{0.6995} & \textbf{0.7676} & \textbf{0.7051} & \textbf{0.7033} & \textbf{0.7054} & \textbf{0.4829} & \textbf{0.1534} & \textbf{0.3392} & \textbf{0.5955} & \textbf{0.3670} & \textbf{0.5459}\\ 
			\bottomrule
			\toprule
			\multirow{4}{*}{Method} & \multicolumn{6}{c|}{{\textbf{Speed Limit}}} & \multicolumn{6}{c}{{\textbf{Road Type}}}  \\
			\cmidrule{2-13}
			& \multicolumn{3}{c|}{{\it Singapore}} & \multicolumn{3}{c|}{{\it Xi'an}} & \multicolumn{3}{c|}{{\it Singapore}} & \multicolumn{3}{c}{{\it Xi'an}} \\
			\cmidrule{2-13}
			& Micro-F1 & Macro-F1 & Weighted-F1 & Micro-F1 & Macro-F1 & Weighted-F1 & Micro-F1 & Macro-F1 & Weighted-F1 & Micro-F1 & Macro-F1 & Weighted-F1 \\ \midrule
			DeepWalk & 0.5784 & 0.1231 & 0.4245 & 0.5820 & 0.5727 & 0.5814 & 0.4987 & 0.2697 & 0.4581 & 0.3697 & 0.2491 & 0.3139\\
			Node2Vec & 0.5782 & 0.1273 & 0.4252 & 0.7661 & 0.7620 & 0.7679 & 0.4984 & 0.2733 & 0.4590 & 0.3791 & 0.2680 & 0.3298\\
			LINE & 0.5781 & 0.1221 & 0.4235 & 0.5920 & 0.6669 & 0.5917 & 0.5059 & 0.2715 & 0.4638 & 0.3892 & 0.2674 & 0.3358\\
			SDNE & 0.5766 & 0.1235 & 0.4243 & 0.4825 & 0.4288 & 0.4546 & 0.4806 & 0.2594 & 0.4422 & 0.3653 & 0.2270 & 0.2940\\
			\midrule
			GAE & \underline{0.5944} & \underline{0.1980} & \underline{0.4654} & 0.7661 & 0.8393 & 0.7636 & 0.5017 & \underline{0.3462} & 0.4762 & 0.4321 & \underline{0.3744} & \underline{0.4097}\\
			GraphSAGE & 0.5910 & 0.1864 & 0.4558 & \underline{0.7711} & \underline{0.8500} & \underline{0.7700} & 0.4955 & 0.3238 & 0.4648 & 0.4312 & 0.3715 & 0.4086\\
			\midrule
			RFN & 0.5904 & 0.1579 & 0.4471 & 0.6368	& 0.6711 & 0.6321 & \underline{0.5260} & 0.3207 & \underline{0.4877} & 0.4031 & 0.2937 & 0.3547\\
			IRN2Vec & 0.5869 & 0.1479 & 0.4341 & 0.6119 & 0.5444 & 0.5962 & 0.4773 & 0.2567 & 0.4353 & 0.3836 & 0.2924 & 0.3475 \\
			HRNR & 0.5868 & 0.1232 & 0.4341 & 0.6915 & 0.6052 & 0.6852 & 0.5050 & 0.2585 & 0.4399 & \underline{0.4485} & 0.3155 & 0.3914\\
			\midrule
			HyperRoad & \textbf{0.6066} & \textbf{0.2534} & \textbf{0.4970} & \textbf{0.7861} & \textbf{0.8566} & \textbf{0.7832} & \textbf{0.5785} & \textbf{0.3964} & \textbf{0.5482} & \textbf{0.4562} & \textbf{0.3957} & \textbf{0.4359}\\ 
			\bottomrule
	\end{tabular}}
	\label{tab:classify}
\end{table*}


\subsection{Performance Comparison (RQ1)} \label{sec:q1}
We first evaluate the learned embeddings in the road segment based tasks. We show the performances of different methods in Table~\ref{tab:classify}, where the best performance is in boldface and the second best is underlined. From the results, we have the following observations. First, the performances of GNN-based methods are generally much better than traditional graph representation learning methods, showing the advantages of deep neural networks in road network structure modelling over shallow representations. Second, the performances of three road network representation learning methods are the best in many cases among the baselines. For example, HRNR tends to perform better on one/two way prediction while RFN is better on road type classification task. IRN2Vec exceeds its counterpart DeepWalk in most cases and the margin reaches near 7\% on one/two way prediction task (\textit{Xi'an}), indicating that the geo-location is one of the key factors in modelling road networks. However, the shallow embedding constrain of IRN2Vec and the simple graph reconstruction objective of RFN and HRNR hinder their performance and superiority on other downstream applications.   
Third, our model performs consistently better than all the baselines in terms of all the metrics on the four tasks. And the average margin in Macro-F1 reaches 18.20\% and 5.18\% for \textit{Singapore} and \textit{Xi'an} dataset respectively. It shows that HyperRoad can better capture the underlying characteristics of road networks with help of the newly neighborhood aggregation mechanism and auxiliary hypergraph-level pre-training task. 

Next, we discuss the model performance on travel time estimation task in Table \ref{tab:tte}. It can be observed that HyperRoad consistently outperforms all competitors on both dataset. The result demonstrates that the road embeddings learned by HyperRoad can also be applicable for traffic level tasks. A possible reason is that the travel time is highly related to road information such as road type and road speed. HyperRoad indeed captures the intrinsic properties of the road networks and thus improve the task performance. It again verifies  the effectiveness of the learned road segment representations from another perspective.

{
\setlength\arrayrulewidth{0.25pt}
\begin{table}[t!]
    \renewcommand{\arraystretch}{1.05} 
	\centering
	\tiny
	\caption{Results for travel time estimation.}
	\label{tab:tte}
	\resizebox{0.78\linewidth}{!}{
		\begin{tabular}{@{}l|cc|cc@{}}
			\toprule[0.35pt]
			\multirow{2}{*}{Method} & \multicolumn{2}{c|}{{\it Singapore}} & \multicolumn{2}{c}{{\it Xi'an}} \\
			\cmidrule[0.25pt]{2-5}
			& MAE & RMSE & MAE  & RMSE  \\ \midrule[0.25pt]
		    DeepWalk & 158.72 & 230.61 & 272.12 & 395.05  \\ 
		    Node2Vec & 152.44 & 219.29 & 272.54 & 390.06 \\
		    LINE & 153.84 & 220.88 & 276.71 & 396.77 \\ 
		    SDNE & 162.43 & 231.80 & 277.62 & 397.26 \\
		    \midrule[0.25pt]
		    GAE & 152.07 & 225.33 & \underline{271.43} & \underline{388.73} \\
		    GraphSAGE & 151.83 & 219.88 & 272.22 & 390.90 \\ 
		    \midrule[0.25pt]
		    RFN & 154.76 & 219.70 & 273.35 & 395.48 \\ 
		    IRN2Vec & \underline{151.45} & \underline{218.06} & 281.89 & 398.86 \\
		    HRNR & 168.35 & 244.09 & 275.62 & 397.22 \\ 
		    \midrule[0.25pt]
		    HyperRoad & \textbf{145.79} & \textbf{214.39} & \textbf{266.50} & \textbf{382.25} \\ 
			\bottomrule[0.35pt]
	\end{tabular}}
\end{table}
\vspace{-0.5cm}
}

\begin{table*}[t!]
	\renewcommand{\arraystretch}{1.25} 
	\centering 
	\caption{Results for ablation studies on Singapore dataset.}
    \normalsize
	\resizebox{1.0\linewidth}{!}{
		\begin{tabular}{c|ccc|ccc|ccc|ccc}
			\toprule
			\multirow{3}{*}{Method} & \multicolumn{3}{c|}{{\textbf{ One/Two Way}}} & \multicolumn{3}{c|}{{\textbf{No. of Lanes}}} & \multicolumn{3}{c|}{{\textbf{Speed Limit}}} & \multicolumn{3}{c}{{\textbf{Road Type}}} \\
			\cmidrule{2-13}
			& Micro-F1 & Macro-F1 & Weighted-F1 & Micro-F1 & Macro-F1 & Weighted-F1 & Micro-F1 & Macro-F1 & Weighted-F1 & Micro-F1 & Macro-F1 & Weighted-F1  \\ \midrule
			w/o PE & 0.7690 & 0.6619 & 0.7421 & 0.4762 & 0.1092 & 0.3091 & 0.5880 & 0.1324 & 0.4420 & \underline{0.5756} & 0.3193 & 0.5301\\
			\midrule
			w/o DAM & 0.7545 & 0.6221 & 0.7164 & 0.4784 & 0.1183 & 0.3145 & 0.5929 & 0.1928 & 0.4544 & 0.5497 & 0.3609 & 0.5114 \\ 
			DAM-ATT & 0.7434 & 0.6079 & 0.7051 & 0.4807 & 0.1339 & 0.3257 & 0.5888 & 0.2001 & 0.4600 & 0.5496 & \underline{0.3789} & 0.5203\\
		    DAM-MLP & 0.7773 & 0.6802 & 0.7545 & 0.4808 & 0.1395 & 0.3295 & 0.5945 & 0.1997 & 0.4653 & 0.5667 & 0.3350 & 0.5255\\
		    \midrule
			w/o GPT  & 0.7804 & 0.6875 & 0.7593 & 0.4793 & 0.1403 & 0.3293 & 0.5876 & 0.1952 & 0.4568 & 0.5742 & 0.3466 & 0.5316\\
			w/o HPT & 0.7402 & 0.5965 & 0.6980 & \underline{0.4827} & 0.1465 & 0.3327 & \underline{0.6016} & \underline{0.2341} & \underline{0.4885} & 0.5220 & 0.3598 & 0.4937\\
		    HyperRoad-DBS  & \textbf{0.7879} & \textbf{0.7017} & \textbf{0.7693} & 0.4796 & \underline{0.1497} & \underline{0.3371} & 0.5962 & 0.2277 & 0.4838 & 0.5724 & 0.3674 & \underline{0.5349}\\
		    \midrule
			HyperRoad & \underline{0.7864} & \underline{0.6995} & \underline{0.7676} & \textbf{0.4829} & \textbf{0.1534} & \textbf{0.3392} & \textbf{0.6066} & \textbf{0.2534} & \textbf{0.4970} & \textbf{0.5785} & \textbf{0.3964} & \textbf{0.5482}\\ 
			\bottomrule
	\end{tabular}}
	\label{tab:ablation}
\vspace{-0.1cm}
\end{table*}

\subsection{Ablation Study (RQ2)}  \label{sec:q2}
In this section, we perform ablation studies on {\it Singapore} dataset to inspect how each module of HyperRoad affects the model performance in four downtream tasks. 

There are three core modules in HyperRoad: positional encoding, dual-channel aggregation mechanism, self-supervised learning with graph-level pretext task and hypergraph-level pretext task. By removing or replacing these modules, we can obtain different variants of HyperRoad. Specifically, we firstly remove the positional encoding module in the model variant w/o PE. Then, we remove the dual-channel aggregation mechanism and obtain the model variant w/o DAM, in which we only use the hyperedge channel aggregation to update the road representations. Note that we do not consider the case of using edge channel aggregation only, since it can not update and output the hyperedge representations necessary for subsequent hypergraph-level objectives. 
In addition, to better validate the design of dual-channel aggregation, we use attention and MLP aggregators in channel fusion and obtain two models named DAM-ATT and DAM-MLP respectively. Finally, models w/o GPT and w/o HPT can be obtained by removing the corresponding graph-level pretext task and hypergraph-level pretext task. We name the model variant using shortest path distance based sampling as HyperRoad-DBS. 
% should be detailed in the method section! Here it is hard to explain the sampling process clearly!
The ablation results are shown in Table \ref{tab:ablation}.

\textbf{Contribution of positional encoding.} By comparing the performance of simplified model w/o PE and full model HyperRoad, we can find that the positional encoding module indeed
brings substantive improvement in downstream task performances. For example, HyperRoad outperforms the base model w/o PE by 40.42\% in Macro-F1 on average. The results justify the fact that the geo-location information is the core property of road network, and it can hardly be captured only by the graph structures. Similar findings can be witnessed in Section \ref{sec:q1} by comparing IRN2Vec and its counterpart DeepWalk. 

\textbf{Contribution of dual-channel aggregation mechanism.} The main difference between HyperRoad and w/o DAM is whether to aggregate information from two channels named edge channel and hyperedge channel at the same time. As seen from the comparative results in Table \ref{tab:ablation}, HyperRoad brings at least 9.83\% improvement in terms of Macro-F1 across all tasks compared with the base model w/o DAM. This is because the two channels capture different graph structure information. Using only one of them will cause information loss and lead to inferior model performance. As for different channel fusion operations, the MLP aggregation performs better on one/two way prediction task while attention aggregation performs better on  road type classification task. However, it is interesting to find that the simple mean aggregation (adopted in HyperRoad) can achieve the best results across all evaluation metrics. A possible reason might be that the extra MLP or attention layer introduces too much non-linearity for road segment embedding learning, which is hard to train and harmful to downstream applications.

\textbf{Contribution of self-supervised pretext tasks.} By com-
paring the performance of w/o GPT, w/o HPT, HyperRoad-DBS and HyperRoad, we can have the following observations. 1) HyperRoad which considers both graph-level and hypergraph-level tasks generally has better performance than the methods considering only single aspect, i.e., w/o GPT and w/o HPT. For example, the full model HyperRoad brings 10.17\% and 14.37\% improvement (in terms of Macro-F1) compared with the base models w/o HPT and w/o GPT on road type classification task. The result demonstrates that both proposed tasks are important for effective road representations. In fact, this conclusion is quit intuitive. For example, it is reasonable that the road segments in a hyperedge (motorways around a lake) might have the same road type (motorways) but slightly different driving speed. Preserving only the hypergraph structure without graph homogeneity constraints may bring noise and lead to biased road representations. 2) By comparing w/o GPT with w/o HPT, we can also find that the model w/o GPT performs better on one/two way and road type classifications while w/o HPT is better on speed limit predictions. From another perspective, it verifies that each task has its own merit to enhance the road segment representations.  3) As for different sampling methods, it is interesting to find that the random sampling method (adopted in HyperRoad) achieves comparable and even better performance than the distance based sampling method. A possible reason is that the location information has already been captured in our model through positional encoding module, and thus the distance based sampling is redundant. Considering the time consuming of pairwise distance calculation, the random sampling is more efficient and applicable for large-scale road network applications. 

\subsection{Parameter Sensitivity (RQ3)}  \label{sec:q3}

We conduct the parameter study on the weighted parameter $\alpha$, the embedding size $d$, and the number of layers $L$ on our example dataset \textit{Singapore} as follows. Fig. \ref{fig:se_analyse} shows the model performance in terms of Macro-F1 under different settings.  

\textbf{The weighted parameter $\alpha$.} As can be seen in Fig. \ref{fig:se_alpha}, the model performances fluctuate with the value of $\alpha$. While HyperRoad remains relatively stable on lanes prediction, it is more sensitive to this parameter in other tasks. Generally, the model performances first increase along with $\alpha$, and then begin to drop when $\alpha$ is larger than 0.1. It is worth mentioning that HyperRoad would reduce to w/o HPT when $\alpha$ is zero, and to w/o GPT when $\alpha$ is infinity. The discovered trend conforms to the their performances in ablation study and again show the necessity of introducing both self-supervised learning tasks.

\textbf{The embedding size $d$.} Fig.~\ref{fig:se_d} shows the impact of embedding size on the results. We can find that the model performances increase with embedding size in most cases, since large embedding size tends to have stronger representational power. However, it is also interesting to discover that using high-dimensional representation does not always produce the best results. For example, the Macro-F1 achieves the best when $d=64$ on road type classification.

\textbf{The number of layers $L$.} As can be seen in Fig. \ref{fig:se_layer}, the model performances remain relatively stable, and the best results for all application tasks can be achieved when $L = 4$. The model performance at $L = 5$ is slightly worse than that of $L = 4$, showing the model capacity is too large and tends to get overfitting and oversmoothing. 

\begin{figure}[t]
	\centering

	\begin{subfigure}[b]{0.42\textwidth}
		\includegraphics[width=\textwidth]{inputs/Figs/road_alpha.pdf}
		\caption{Parameter $\alpha$ (\textit{Singapore})}
		\vspace{0.3cm}
		\label{fig:se_alpha}
	\end{subfigure}
	
	\begin{subfigure}[b]{0.42\textwidth}
		\includegraphics[width=\textwidth]{inputs/Figs/road_emb.pdf}
		\caption{Parameter $d$ (\textit{Singapore})}
		\vspace{0.3cm}
		\label{fig:se_d}
	\end{subfigure}

	\begin{subfigure}[b]{0.42\textwidth}
		\includegraphics[width=\textwidth]{inputs/Figs/road_layer.pdf}
		\caption{Parameter $L$ (\textit{Singapore})}
		\label{fig:se_layer}
	\end{subfigure}
	\caption{Impact of hyper-parameters $\alpha$, $d$ and $L$ on model performances.}
    \label{fig:se_analyse}
\vspace{-0.5cm}
\end{figure}



\begin{figure*}[t!]
	\centering
    \begin{subfigure}[b]{0.18\textwidth}
		\includegraphics[width=\textwidth]{inputs/Figs/DeepWalk.pdf}
		\caption{DeepWalk}
		\label{fig:dw}
	\end{subfigure}
	\hspace{0.01\textwidth}
	\begin{subfigure}[b]{0.18\textwidth}
		\includegraphics[width=\textwidth]{inputs/Figs/Node2Vec.pdf}
		\caption{Node2Vec}
		\label{fig:nodev}
	\end{subfigure}
	\hspace{0.01\textwidth}
	\begin{subfigure}[b]{0.18\textwidth}
		\includegraphics[width=\textwidth]{inputs/Figs/LINE.pdf}
		\caption{LINE}
		\label{fig:line}
	\end{subfigure}
	\hspace{0.01\textwidth}
	\begin{subfigure}[b]{0.18\textwidth}
		\includegraphics[width=\textwidth]{inputs/Figs/SDNE.pdf}
		\caption{SDNE}
		\label{fig:sdne}
	\end{subfigure}
	\hspace{0.01\textwidth}
	\begin{subfigure}[b]{0.18\textwidth}
		\includegraphics[width=\textwidth]{inputs/Figs/IRN2Vec.pdf}
		\caption{IRN2Vec}
		\label{fig:irn}
	\end{subfigure}
	
    \vspace{0.02\textwidth}
    
	
	\begin{subfigure}[b]{0.18\textwidth}
		\includegraphics[width=\textwidth]{inputs/Figs/HRNR.pdf}
		\caption{HRNR}
		\label{fig:hrnr}
	\end{subfigure}
	\hspace{0.01\textwidth}
	\begin{subfigure}[b]{0.18\textwidth}
		\includegraphics[width=\textwidth]{inputs/Figs/RFN.pdf}
		\caption{RFN}
		\label{fig:rfn}
	\end{subfigure}
    \hspace{0.01\textwidth}
	\begin{subfigure}[b]{0.18\textwidth}
		\includegraphics[width=\textwidth]{inputs/Figs/GraphSAGE.pdf}
		\caption{GraphSAGE}
		\label{fig:sage}
	\end{subfigure}
	\hspace{0.01\textwidth}
	\begin{subfigure}[b]{0.18\textwidth}
		\includegraphics[width=\textwidth]{inputs/Figs/GAE.pdf}
		\caption{GAE}
		\label{fig:gae}
	\end{subfigure}
	\hspace{0.01\textwidth}
	\begin{subfigure}[b]{0.18\textwidth}
		\includegraphics[width=\textwidth]{inputs/Figs/Hyper.pdf}
		\caption{HyperRoad}
		\label{fig:hyper}
	\end{subfigure}
	
	\caption{Road segment embedding visualizations for the studied area. Color of a node indicates its road type. Green: "motorway", Red: "residential".}
	\label{fig:embedding}
\end{figure*}

\begin{figure}[t]
	\centering

	\begin{subfigure}[b]{0.24\textwidth}
		\includegraphics[width=\textwidth]{inputs/Figs/case_1.pdf}
		\caption{Case one: $r5028$}
		\vspace{0.2cm}
		\label{fig:se_alpha}
	\end{subfigure}
	\begin{subfigure}[b]{0.24\textwidth}
		\includegraphics[width=\textwidth]{inputs/Figs/case_2.pdf}
		\caption{Case two: $r30396$}
		\vspace{0.2cm}
		\label{fig:se_d}
	\end{subfigure}
	\caption{Road segment similarity visualizations.}
	\label{fig:simi}
\vspace{-0.5cm}
\end{figure}

\begin{table}[t!]
	\renewcommand{\arraystretch}{1.25} 
	\centering 
	\caption{A show case of road segment similarity.}
    \normalsize
	\resizebox{1.0\linewidth}{!}{
		\begin{tabular}{c|ccccc|ccccc}
			\toprule
			\multirow{3}{*}{Category} & \multicolumn{5}{c|}{{\textbf{ Case One}}} & \multicolumn{5}{c}{{\textbf{Case Two}}} \\
			\cmidrule{2-11}
			& Road ID & One/Two Way & No. of Lanes  & Speed Limit & Road Type & Road ID & One/Two Way & No. of Lanes  & Speed Limit & Road Type  \\ \midrule
			Target road & $r5028$ & one way & 3 & 90 & motorway & $r30396$ & two way & 2 & 50 & residential \\
			\midrule
			\multirow{5}{*}{Similar roads by GAE} & $r6832$ & one way & 4 & 90 & motorway & $r2133$ & two way & 2 & 50 & residential \\
			& $r16803$ & one way & 3 & 90 & motorway & $r21127$ & one way & 1 & 50 & motorway  \\ 
			& $r5027$ & one way & 2 & 50 & motorway & $r5514$ & one way & 1 & 50 & motorway  \\ 
			& $r16804$ & one way & 2 & 50 & motorway & $r5995$ & one way & 1 & 50 & motorway \\
			& $r6831$ & one way	& 1 & 50 & motorway & $r27877$ &	one way & 1 & 50 & motorway  \\ 
			\midrule
			\multirow{5}{*}{Similar roads by HyperRoad} & $r16803$ & one way & 3 & 90 & motorway & $r6328$ & two way & 2 & 50 & residential \\
			& $r28968$ & one way & 3 & 90 & motorway & $r2133$ & two way & 2 & 50 & residential \\
			& $r25372$ & one way & 4 & 90 & motorway & $r32071$ & two way & 2 & 50 & residential \\
			& $r6832$ & one way & 4 & 90 & motorway & $r9356$ & two way & 2 & 50 & residential \\
			& $r3221$ & one way & 4 & 70 & motorway & $r29281$ & two way & 2 & 50 & residential \\
			\bottomrule
	\end{tabular}}
	\label{tab:simi}
\vspace{-0.3cm}
\end{table}

\subsection{Case Study for Representation Understanding (RQ4)}  \label{sec:q4}
In this section, we use auxiliary information such as road segment attributes to help uncover what HyperRoad is learning. Note that these information is not available for our model training.

We first exploit the network visualization approach to evaluate node embeddings learned by different methods. Here, we take a rectangular region of \textit{Singapore} as an example. The longitude is between $103^\circ 77^\prime \text{E}$ and $103^\circ 84^\prime \text{E}$, and the latitude is between $1^\circ 33^\prime \text{N}$ and $1^\circ 43^\prime \text{N}$. Then, we select road segments located in this region and employ the t-SNE method \cite{van2008visualizing} to project road embeddings to a 2-dimensional space. For the sake of visualization, we present the results for two road types with different semantics namely motorway and residential. 
% There are 1592 points for residential class and 1270 points for motorway. 
The projected results of different methods are shown in Fig. \ref{fig:embedding}, using the color and shape of a node to indicate its road type. From the results, we make the following observations. 1) The shallow network representation methods failed to separate the two road types clearly. For example, in DeepWalk, two road types are mixed together in the middle of Fig. \ref{fig:dw}. Although IRN2Vec considers the geo-location and shape information in road network compared with DeepWalk, it still can not achieve satisfactory visualizing results as shown in Fig. \ref{fig:irn}. The reason is that random walks may not preserve the node homogeneity, and thus lead to similar representations for road segments with different semantics. 2) There are different clusters in the results of HRNR as shown in Fig. \ref{fig:hrnr}. This is because HRNR is a hierarchical GNN structure, and each node can aggregate information from too many neighbors through the hidden nodes. This aggregation mechanism leads to the oversmoothing problem. 3) RFN, GraphSAGE and GAE provide better performance than other baselines and obtain more reasonable visualizing results. However, some clusters are still mixed with each other and there is no clear margin between different classes. 4) In contrast, HyperRoad gives the most satisfying identification with relatively clear cluster boundaries, which demonstrates that the road functionalities are well preserved by our model. The reason is that the proposed dual-channel aggregation mechanism can help the model to find long-range neighbors with similar semantics, and the hypergraph-level tasks provides extra semantic constrains and domain knowledge for road representation learning. 

We further pick two specific cases to explain the road embeddings learned by different methods in details. GAE is selected as a reference method because of its satisfactory task performances and visualizing results. 
Specifically, we first randomly sample two road segments $r5028$ and $r30396$ with distinct semantic information as target roads. For each road segment, we extract its top 5 most similar roads in GAE and HyperRoad with cosine similarity. The road attributes information is shown in Table \ref{tab:simi} and the geo-location information is plotted in Fig. \ref{fig:simi}. It is clear to see that GAE mainly recalls very close neighbors in spatial position although their attributes are different. For example, in case one, the ramp is taken as the similar road segment for the target road with higher speed. And the motorways are considered similar to residential road segment in case two. The results show that the adopted graph reconstruction objective is not effective enough in modelling complex road networks. In contrast, our model considers both spatial and semantic information together when querying similar road segments. For example, in both case one and case two, our model can find the road segments with similar functions in a reasonable long range, which justifies the necessity of the proposed hyperedge modeling.

\if 0 
\begin{figure}[t!]
	\centering
	\includegraphics[width=0.2\textwidth]{inputs/Figs/plot_case.pdf}
	\caption{A show case of the studied area.}
	\label{fig:area}
\end{figure}
\fi


==> inputs/experiment_setting.tex <==
\section{Experimental Setup}
\label{sec:expsetup}

In order to show the effectiveness of our proposed model HyperRoad, we conduct extensive experiments to answer the following questions.

RQ1: Can HyperRoad outperforms other methods on the downstream tasks when only structure and position information is available (the most generic setting in real world)?

RQ2: What roles do different components of HyperRoad play in improving the model performance?

RQ3: How would different hyper-parameters influence the model results of HyperRoad?

RQ4: What do the learned road embeddings represent? Can these embeddings capture the underlying characteristics of road networks?

RQ5: Can HyperRoad outperforms the state-of-the-art methods under different settings?

%Aiming at answering these important questions, we use 2 real-world road network datasets, and also adopt 9 different baselines on 5 downstream tasks, including both road segment based and trajectory based applications, for comparisons. 
In this section, we first describe the detailed experimental settings.

\subsection{Datasets}
We use the road networks and trajectories of two cities, Singapore and Xi'an in the experiments. The road networs are extracted from OpenStreetMap \footnote{https://www.openstreetmap.org/}, and the trajectories are obtained from public datasets released by DiDi Chuxing \footnote{https://www.didiglobal.com} and Grab \footnote{https://www.grab.com/sg/} \cite{huang2019grab}. The Singapore trajectory dataset is sampled every second, while the Xi'an dataset is sampled every 2-4 seconds. Note that the trajectory dataset is only used in downstream applications to evaluate the model performance  but not used in pre-training stage.
We then apply map segmentation algorithm \cite{yuan2012discovering} on each road network to construct hypergraphs as detailed in Section \ref{sec:pf}. 
% need explanation in previous sections, how to segment and how to construct the hypergraph.
The statistics of these datasets are shown in Table \ref{tab:data}.

{
\setlength\arrayrulewidth{0.30pt}
\begin{table}[t!]
	\renewcommand\arraystretch{1.15}
	\centering
	\caption{Statistics of the datasets.}
	\scriptsize
    
	\resizebox{0.75\linewidth}{!}{
		\begin{threeparttable}
			\begin{tabular}{c|c|c}
				\toprule[0.38pt]
				Dataset & Singapore &  Xi'an  \\
				\midrule[0.30pt]
				\# Road Segments & 33948 & 53067 \\  
				\# Hyperedges & 3772 & 6953 \\
				\# Road-Road & 147550 & 249848 \\ 
				\# Road-Hyperedge & 54031 & 86301 \\ 
				\# Trajectories & 28000 & 50000 \\ 
				\bottomrule[0.38pt]
			\end{tabular}
		\end{threeparttable}}
	\label{tab:data}
\end{table}
}

\subsection{Baseline Methods}
We compare our proposed method HyperRoad with the following 9 baselines, namely DeepWalk \cite{perozzi2014deepwalk}, Node2Vec \cite{grover2016node2vec}, LINE \cite{tang2015line}, SDNE \cite{wang2016structural}, GAE \cite{kipf2016variational}, GraphSAGE \cite{hamilton2017inductive}, RFN \cite{jepsen2020relational}, IRN2Vec \cite{wang2019learning} and HRNR \cite{wu2020learning}. Among them, DeepWalk, Node2Vec, LINE and SDNE are traditional graph representation learning methods; GAE and GraphSAGE are newly GNN-based graph representation learning methods; and RFN, IRN2Vec and HRNR are the recent representation learning methods designed for road networks. Note that another road network representation learning method Toast \cite{chen2021robust} will degrade to DeepWalk when trajectory and road context information are not available in pre-training stage, which is the common situation for larger-scale road networks.

Following the existing works \cite{jepsen2020relational, wang2019learning, wu2020learning}, We do not consider the specialized methods which are designed for a specific task as baselines, because our goal is to evaluate the usefulness and generalization of the learned road representations. Thus we use the same task-specific components and make them as simple as possible for all the compared methods. Using specialized methods is not a fair comparison here. 

% Details of these baseline and their parameter settings are provided as follows.
These baseline methods and their parameter settings are briefly introduced as follows. Note that the positional encoding mechanism is also used in baselines for fair comparison. 

\begin{itemize}[leftmargin=*]
  \item \textbf{DeepWalk \cite{perozzi2014deepwalk}}: It transforms the network into node sequences by uniform random walks, and then learns node representations through skip-gram model. The walk length and the window size are set to be 20 and 5 respectively. The number of walks per node are searched in \{30, 50, 80\}.
  \item \textbf{Node2Vec \cite{grover2016node2vec}}: It is an extension of DeepWalk and adopts a biased random walk to generate node sequences. The number of walks, the walk length and the window size are tuned in the same way with DeepWalk. The parameters $p$ and $q$ for biased random walk are tuned in \{0.25, 0.5, 1.0, 2.0\}.
  \item \textbf{LINE \cite{tang2015line}}: It learns node representation by considering both first and second order node proximities. We use half dimensions to capture the first-order proximity, and another half dimensions to capture the second-order information. 
  \item \textbf{SDNE \cite{wang2016structural}}: It represents the network as an adjacency matrix, and obtains node embeddings through autoencoder. The encoder and decoder are implemented as a two-layer MLP with hidden dimensions of \{1024, 64\}.
  \item \textbf{GAE \cite{kipf2016variational}}: It extends the idea of SDNE by using graph convolutional network (GCN) to learn node representations. The number of GCN layers for GAE is selected from \{2, 3, 4\}.
  \item \textbf{GraphSAGE \cite{hamilton2017inductive}}: It is another GNN based unsupervised graph representation learning method. We use mean aggregator and tune the number of GNN layers in the set of \{2, 3, 4\}.
  \item \textbf{RFN \cite{jepsen2020relational}}: It learns road segment representations based on dual node-relational and edge-relational views. The messages are passed and interacted in both views and the training objective is network reconstruction. The number of GNN layers is tuned the same with GraphSAGE. 
  \item \textbf{IRN2Vec \cite{wang2019learning}}: IRN2Vec is road network representation method developed based on DeepWalk. It replaces the uniform random walk with shortest path sampling, and applies skip-gram model to predict the information of geo-locality, geo-shape, and road tags given road sequences. We adapt this method by excluding the road tags information which is not available in our setting. The parameters are set the same as that in DeepWalk.
  \item \textbf{HRNR \cite{wu2020learning}}: It learns road representation by preserving different levels of road network semantic information in a hierarchical manner. We follow the experiment settings in the original paper but excluding the top level because it is based on trajectory information, which suffers from coverage and availability problems and is no available in our setting.
\end{itemize}

\subsection{Application Tasks}
We consider using two types of downstream applications for testing the effectiveness of learned road representations, including road segment based and trajectory based applications. 
For each task, we employ a simple task-specific components (\textit{e.g.}, LSTM or Logistic Regression) with the learned road network representations as input to perform predictions. As mention above, we exploit the same task-specific components for all the methods for fair comparison. The adopted application tasks are described as follows:

\textbf{Road segment based tasks.} Following the existing work \cite{yin2021multimodal}, we consider the following four important road attribute predictions as road segment based tasks: 1) one/two way classification, 2) lanes classification, 3) speed limit classification, and 4) road type classification. 
For each task, we choose the road attribute values as the labels, regard the learned road segment representations as input features, and use a one-vs-rest logistic regression classifier to make predictions. 

\textbf{Trajectory based tasks.} Following the existing work \cite{wang2019learning}, we use another travel time estimation task to further verify the effectiveness and ubiquity of the road embeddings learned by HyperRoad. Travel time estimation is a regression task to predict the travel time of a given moving path in road networks. Thus, we firstly perform map matching \cite{yang2018fast} by aligning the raw GPS points with road networks to transform the raw trajectory data into road segment sequences. The ground truth is also extracted as the time difference between the first and last GPS point (in seconds).
Then, we apply a simple Long Short-Term Memory (LSTM) layer followed by one fully-connected layer as the regression model, which takes the road segment representation as input and outputs the estimated travel time. 

\subsection{Evaluation Metrics}
We adopt different evaluation metrics for the above two different types of tasks. 

For road segment based tasks, Micro-F1, Macro-F1 and Weighted-F1 are used to evaluate the classification accuracy. Among them, the Micro-F1 computes a global average F1 score by counting the sums of the True Positive (TP), False Positive (FP), and False Negative (FN) of each class, while the Macro-F1 is computed by taking the arithmetic mean of all the per-class F1 scores. Finally, the Weighted-F1 score is obtained by taking the mean of all per-class F1 scores while considering each class’s support.

For trajectory based tasks (travel time estimation), MAE (Mean Average Error) and RMSE (Root Mean Square Error) are used to measure the closeness between the predicted value and the real value. Among them, MAE measures the average absolute distance between predictions and ground-truths, and RMSE measures the average quadratic errors of all predictions.

\subsection{Parameter Setting}
In our experiments, we set the embedding dimension to be 64 for all the methods for fair comparison. We use a mini-batch Adaptive Moment Estimation (Adam)~\cite{kingma2015adam} optimizer to train HyperRoad. The learning rate and batch size are set to be 0.001 and 1024 respectively. The scale parameter $\phi$ and frequency parameter $\lambda$ in Equation \ref{eq:pe} are set to be 10 and 1000 separately. The weighted parameter $\alpha$ in the loss function is set to be 0.1 for both datasets. The negative sizes for graph sampling and hypergraph sampling named $N_G$ and $N_H$ are set to be 5 and 2 respectively. The number of hyperedge clusters are set to be 8 and 7 for Singapore dataset and Xi'an dataset. We also tune the number of layers in the set of \{2,3,4\}.



==> inputs/introduction.tex <==
\section{Introduction} \label{sec:intro}
As the fundamental component of the transportation systems, road network is closely related to numerous downstream transportation applications, including traffic based tasks such as traffic inference and forecasting \cite{guo2019attention}, and road segment based tasks such as road tag prediction \cite{yin2021multimodal}. Due to its important role, studying the road network representations can help us explore the functions and properties of transportation systems, and directly boost the effectiveness of all these tasks. Since a road network is essentially a special graph, recent works have proposed to utilize various graph representation learning methods to address this problem. These methods can be roughly divided into two categories named random walk based and GNN based methods. 

Random walk based methods such as DeepWalk \cite{perozzi2014deepwalk} and Node2Vec \cite{grover2016node2vec} are the earliest attempts in graph representation learning. They borrow the idea of word representation \cite{mikolov2013distributed} into graph data, and regard the node sequences generated by random walks as sentences. Then skip-gram model can be used to learn node representations. Following a similar idea, IRN2Vec \cite{wang2020representation, wang2019learning} is proposed to model road networks by considering extra geo-location and shape information when sampling node sequences. While these methods can be applied to learn road network representations, they are not effective due to the following two issues: ($\mathbf{i}$) \textit{Shallow Representation}. All these methods are actually equivalent to the matrix factorization framework \cite{qiu2018network}, where the node encoder is a simple embedding lookup table. However, deep architectures have been proven important for effective representation extraction \cite{bengio2013representation}. Meanwhile, the scheme also limits the potential to integrate extra information if available. ($\mathbf{ii}$) \textit{Noise in Random Walk}. The representations of these methods depend heavily on the quality of input node sequences. Unfortunately, these node sequences are generated by random walks on graph, which may introduce noises. For example, the motorway road and residential road can co-occur frequently in a random path and thus lead to mixed representations. 

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.38\textwidth]{inputs/Figs/intro_case.pdf}
	\caption{Road network example.}
	\label{fig:intro}
	\vspace{-0.5cm}
\end{figure}

Recent years have witnessed the success of graph neural networks (GNNs) in modeling graph data \cite{kipf2016semi, velivckovic2017graph, xu2018powerful}. The core procedure of GNNs is to perform message passing and aggregation from neighborhoods. Some existing works such as RFN and HRNR  \cite{jepsen2020relational, wu2020learning} have adopted GNN into unsupervised road network representation problem by optimizing a graph reconstruction pretext task. Despite GNNs achieve relatively satisfactory results, they still suffer from two limitations in road network setting:  ($\mathbf{i}$) \textit{Expressive Power.} Existing GNN-based methods mainly focus on pairwise node interactions. However, the function of road segments may not be captured by simple dyadic relations but high-order interactions. For instance, considering "Road A" as an example, if we adopt the simple graph to model road networks, GNNs may misinterpret its function and generate incorrect representations because "Road A" has more pairwise connections with walk roads. However, if we consider higher-order relations in the context of the entire highway loop such as the other two red road segments jointly (\textit{i.e.} triadic relations), the actual meaning of "Road A" can be better modeled. Therefore, how to go beyond pairwise relationships and further capture high-order road segment interactions is crucial for high-quality road network representation, but remains to be explored. ($\mathbf{ii}$) \textit{Long Range Correlations.} Neighborhood aggregation and graph reconstruction are two core components in existing GNN based representation learning methods for road networks. However, both mechanisms are difficult to deal with the long range correlations problem in road network. For example, "Road B" and "Road C" are two road segments that share similar information, despite being far apart on the map. From the view of GNNs, a conclusion of no direct correlation is usually made and thus lead to information loss. Hence, it is necessary to design an approach to model such semantic dependencies explicitly. 

To address these challenges, we introduce hypergraph (a hypergraph is a more general topological structure than simple graph where a hyperedge could connect two or more nodes) in road networks, and propose a general representation learning framework called HyperRoad (\underline{Hyper}graph-Oriented \underline{Road} network representation). The use of hypergraphs enable our model capture high-order contextual information of each road segment beyond pairwise interactions. Based on that, a new neighborhood aggregation operation named dual-channel aggregating mechanism is further proposed to boost expressive power. To tackle the long range correlation challenge, we propose to use hypergraph as information medium for correlation propagation, and propose a novel scheme named bi-level self supervised learning. Due to the inadequacy of simple graph reconstruction on road network settings, we design both graph-level and hypergraph-level pretext tasks in this module for learning highly expressive representations, where each part can provide complementary supervision signals. 
To summarize, our contributions are in three-fold:
\begin{itemize}
\item  For the first time, we propose to model road networks as hypergraphs, and design novel hypergraph construction strategies on road network.
\item We propose a novel road network representation learning framework called HyperRoad, which is featured with a hypergraph based dual-channel aggregation module to model high-order road relations and enhance model expressive power, and a bi-level self-supervised learning module to provide complementary supervision signals and capture both local and global road correlations.
\item We conduct extensive experiments on five downstream applications including both road segment based and trajectory based, and the results  demonstrate that our model outperforms existing methods across all these tasks.
\end{itemize}

==> inputs/method.tex <==
\section{METHODOLOGY} \label{sec:model}

\begin{figure*}[t!]
	\centering
	\includegraphics[width=0.95\textwidth]{inputs/Figs/Frame_Hyper.pdf}
	\caption{The architecture of HyperRoad.}
	\label{fig:framework}
\vspace{-0.3cm}
\end{figure*}

{\CHENG{In this section, we propose a novel model called HyperRoad for road network representation learning (RNRL). The overview of the model architecture is shown in Fig. \ref{fig:framework}. HyperRoad is based on three key ideas: (1) it constructs a \emph{hypergraph}, where each hyperedge corresponds to a set of multiple roads forming a region, (2) it propagates information via both edges (of a simple graph capturing the pairwise relationships) and hyperedges (of the constructed hypergraph) in a context of graph neural network, and (3) it optimizes the road representations with a few pretext tasks based on both the simple graph (i.e., graph reconstruction) and the constructed hypergraph (including hypergraph reconstruction and hyperedge classification).}}
% In this section, we detail the basic model HyperRoad for road network representation learning problem by considering pure road network structures and geo-locations. The overview of the model architecture is shown in Fig. \ref{fig:framework}. Firstly, to cope with the expressive power issue of existing methods, we propose to construct hypergraph which can connect arbitrary number of road segments naturally, and design a new dual-channel aggregation module to capture high-order contextual information instead of the pairwise modelling. Secondly, to deal with the long range correlation problem, we find that the hyperedge can transfer knowledge across road segments far apart on the map, and design two novel hyperedge based self supervised training tasks for road network setting beyond simple graph reconstruction. 

\subsection{Position-aware Embedding Generation}
To represent the innate geo-spatial information in road networks, we follow the strategy in BERT \cite{devlin2018bert} to jointly embed the road segment and its location into dense representations as the model inputs.
Specifically, for each road segment $v_i$, we first encode it with an embedding vector $\mathbf{q}_i$. All road segment embeddings are represented as an embedding matrix $\mathbf{Q} \in \mathbb{R}^{d}$, which will be learned in an end-to-end manner.

Then, motivated by recent advances in transformers \cite{devlin2018bert} and spatial representation learning \cite{mai2020multi}, we propose a positional encoder module to model spatial context information. In specific, given the coordinates vector $\mathbf{p}_i$ for road segment $v_i$, we use sine and cosine functions of different frequencies to generate the positional encoding $\mathbf{u}_i$ as follows,

\begin{equation}
\label{eq:pe}
%PE(\mathbf{p}_i) = 
\left\{
    \begin{aligned}
        & \textbf{u}_i(4k) = sin((\textbf{p}_i^{[0]}/\phi) / \lambda^{4k/d}), \\
        & \textbf{u}_i(4k+1) = cos((\textbf{p}_i^{[0]}/\phi) / \lambda^{4k/d}), \\
        & \textbf{u}_i(4k+2) = sin((\textbf{p}_i^{[1]}/\phi) / \lambda^{4k/d}), \\ 
        & \textbf{u}_i(4k+3) = cos((\textbf{p}_i^{[1]}/\phi) / \lambda^{4k/d}),
    \end{aligned} \right. 
\end{equation}

where $k$ denotes the $k$-th dimension, $d$ denotes the embedding size, $\textbf{p}_i^{[0]}$ and $\textbf{p}_i^{[1]}$ denotes the projected latitude and longitude values. $\phi$ is the scale parameter to constrain the size of projected values, and $\lambda$ is the frequency parameter similar to positional encoding in transformers. We extend 1D discrete positions in NLP to 2D continuous positions in geospace.

Finally, for each road segment $v_i$, we fuse its embedding and positional embedding into a single one as follows.

\begin{equation}
\label{eq:input}
\mathbf{r}_i = \text{MLP}(\mathbf{q}_i \mathbin\Vert \mathbf{u}_i),
\end{equation}

where $\mathbin\Vert$ is the concatenate operation and $\text{MLP}$ is a fully connected neural network. 

\subsection{Dual-channel Aggregating Mechanism}
In this module, we describe our embedding aggregation scheme, which iteratively aggregates the information from related road segments to encode the structures. Given the road network $\mathcal{G_R}$ and hypergraph $\mathcal{G_H}$, it is obvious that the edge level neighborhoods in $\mathcal{G_R}$ provide pairwise modelling and local receptive fields, and the hyperedge level neighborhoods in $\mathcal{G_H}$ endows the potential to model the complex high-order dependencies. Both kinds of information are indispensable and complementary for road segment modelling. For example, the hyperedge context (\textit{e.g. highway ring}) and local environment (\textit{e.g. residential area}) can jointly determine the function of a ramp road. Therefore, we summarize the message aggregation into two channels, \textit{i.e.}, edge channel and hyperedge channel and devise a novel dual-channel aggregating mechanism. We first illustrate the design of one-layer aggregation and then generalize it to multiple layers.

\textbf{Edge Channel Aggregation.} The goal of this sub-module is to propagate node information from graph contexts. This process can be formulated as:

\begin{equation}
	\mathbf{h}_{i \gets edge}^{(l)} = AGG(\{\mathbf{h}_{j}^{(l)}, \, v_j \in \mathcal{N}_i\}),
\end{equation}

where $\mathbf{h}_{i \gets edge}^{(l+1)}$ is the message received by node $v_i$ from edge channel, $l$ represents the layer number, $\mathcal{N}_i$ denotes the neighborhoods of node $v_i$ defined by edges in  $\mathcal{G_R}$. When $l=0$, $\mathbf{h}_{i}^{(0)}$ is set to be the position-aware input embedding $\mathbf{r}_i$ for node $v_i$. $AGG(\cdot)$ is an aggregation function, which is implemented as a mean aggregator in this paper to keep the model simple. 
%Note that other kinds of operations such as attention aggregator \cite{velivckovic2017graph} 
% and bilinear interaction aggregator \cite{zhu2020bilinear} can also be adopted in our framework without changing the model structures.  

\begin{equation}
	\mathbf{h}_{i \gets edge}^{(l)} = \text{ReLU} ( \frac{1}{|\mathcal{N}_i|} \sum_{v_j \in \mathcal{N}_i} \, \mathbf{W}_{1}^{(l)} \mathbf{h}_{j}^{(l)} ),
\end{equation}

where $\mathbf{W}_{1}^{(l)}$ is the trainable weight matrix to distill
useful information for propagation and the normalization term $1 / |\mathcal{N}_i|$ is to constrain the embedding scales.

\textbf{Hyperedge Channel Aggregation.} In addition to edge aggregations, HyperRoad learns node representations through hypergraph convolutions,  allowing to capture high-order context information of road segment to enhance the model representation ability. Specifically, we define our hyperedge channel aggregation by using the following two-step operations. 
\begin{equation}
\begin{aligned}
	\mathbf{m}_{j}^{(l)} = AGG(\{\mathbf{h}_{i}^{(l)}, \, v_i \in \mathcal{R}_j\}), \\ 
	\mathbf{h}_{i \gets hyper}^{(l)} = AGG(\{\mathbf{m}_{j}^{(l)}, \, e_j \in \mathcal{H}_i\}),
\end{aligned}
\end{equation}

where $\mathcal{R}_j$ denotes the set of nodes connected to hyperedge $e_j$ in $\mathcal{G_H}$,  and $\mathbf{m}_{j}^{(l)}$ is the aggregated hyperedge representation of $e_j$. $\mathcal{H}_i$ represents the neighbor hyperedge set of node $v_i$ such that $\mathbf{H}_{i,j} = 1$, and $\mathbf{h}_{i \gets hyper}^{(l)}$ is the message received by node $v_i$ from hyperedge channel. The proposed two-step information propagation scheme performs ‘node-hyperedge-node’ feature transformation upon hypergraph structure, and the hyperedge acts as an information medium during this process. In this paper, we simply implement those two $AGG(\cdot)$ functions by mean aggregators to avoid extra model parameters as follows. 
% We leave the exploration of other operations to future work.

\begin{equation}
\begin{aligned}
	\mathbf{m}_{j}^{(l)} = \text{ReLU} ( \frac{1}{|\mathcal{R}_j|} \sum_{v_i \in \mathcal{R}_j} \, \mathbf{W}_{2}^{(l)} \mathbf{h}_{i}^{(l)} ), \\ 
	\mathbf{h}_{i \gets hyper}^{(l)} = \text{ReLU} ( \frac{1}{|\mathcal{H}_i|} \sum_{e_j \in \mathcal{H}_i} \, \mathbf{W}_{3}^{(l)} \mathbf{m}_{j}^{(l)} ),
\end{aligned}
\end{equation}
where $\mathbf{W}_{2}^{(l)}$ and $\mathbf{W}_{3}^{(l)}$ are feature transformation matrices at different granularities.

\textbf{Channel Fusion.} In this stage, we aggregate all the messages to update the node representations. Apart from aggregating information from other nodes, we also add a residual connection here motivated by \cite{devlin2018bert}
%\cite{he2016deep, vaswani2017attention} 
to preserve node's own features and help model training. We name this information channel as self channel, and it copies node embeddings directly to the next layer. Taking node $v_i$ as an example, we will have message vector $\mathbf{h}_{i \gets self}^{(l)} = \mathbf{h}_{i}^{(l)}$. Formally, the new representation of $v_i$ can be formulated as follows.

\begin{equation}
	\mathbf{h}_{i}^{(l+1)} = f( \ \underbrace{\mathbf{h}_{i \gets self}^{(l)}}_{\text{self channel}}, \underbrace{\mathbf{h}_{i \gets edge}^{(l)}}_{\text{edge channel}}, \underbrace{\mathbf{h}_{i \gets hyper}^{(l)}}_{\text{hyperedge channel}}). 
\end{equation}

In this work, we implement $f(\cdot)$ using the following three types of functions:

\begin{itemize}[leftmargin=*]
  \item \textit{Mean Fusion} averages the messages from the three channels as output without trainable parameters. 
  
    \begin{equation}
    	f_{mean} = (\mathbf{h}_{i \gets self}^{(l)} + \mathbf{h}_{i \gets edge}^{(l)} + \mathbf{h}_{i \gets hyper}^{(l)} ) / 3.
    \end{equation}
    
    \item \textit{Attention Fusion} learns message importance through attention mechanism and regards  output as the weighted sum of messages. 
    
    \begin{equation}
    f_{att} = \theta_s \cdot \mathbf{h}_{i \gets self}^{(l)} + \theta_e \cdot \mathbf{h}_{i \gets edge}^{(l)} + \theta_h \cdot \mathbf{h}_{i \gets hyper}^{(l)}.
    \end{equation}
    Without loss of generality, we take the weight $\theta_s$ as an example. It is defined as:
    
    \begin{equation}
    \begin{aligned}
    \tilde{\theta}_{s} = \text{MLP}(\mathbf{h}_{i \gets self}^{(l)}), \ \theta_{s} = \frac{\exp(\tilde{\theta}_{s})}{\sum_{c \in \{s,e,h\}} \exp(\tilde{\theta}_{c})}. 
    \end{aligned}
    \end{equation}
  
    \item \textit{MLP Fusion} concatenates all messages, followed by a fully connected neural network.
    
    \begin{equation}
    	f_{mlp} = \text{MLP}(\mathbf{h}_{i \gets self}^{(l)} \mathbin\Vert \mathbf{h}_{i \gets edge}^{(l)} \mathbin\Vert \mathbf{h}_{i \gets hyper}^{(l)}).
    \end{equation}
  
\end{itemize}
In this paper, we use $f_{mean}$ as the default model design in HyperRoad and empirically compare the three fusions in Section \ref{sec:q2}.

With the representations augmented by direct neighborhoods modeling, we further consider to stack aforementioned aggregation module to $L$ layers such that the model receptive fields are enlarged. Specifically, we name the node and hyperedge representations for $v_i$ and $e_j$ in the last layer as $\mathbf{h}_i$ and $\textbf{m}_j$ respectively. 

\subsection{Bi-level Self Supervised Learning}
It is usually the case that a well-designed loss function plays a vital role in achieving desired properties for pre-training models in various domains.
% such as natural language processing \cite{devlin2018bert} and computer vision  \cite{lu2019vilbert}. 
To this end, we design two types of pretext tasks in road network setting, \textit{i.e.}, graph-level and hypergraph-level tasks to effectively encode the road network structures into representations. 

\textbf{Graph-level Pretext Task.} To let the learned road embeddings reserve the adjacent correlations between road segments in $\mathcal{G_R}$, we design the first pretext task named \textit{graph reconstruction} to reconstruct adjacency matrix $\mathbf{A}$ based on corresponding embeddings. Specifically, we maximize the probability of connected road pairs as:

\begin{equation}
\begin{aligned}
    \mathcal{L}_{GR} = - \sum_{v_i \in \mathcal{V}} \sum_{v_j \in \mathcal{N}_i} \left(\mathbf{h}_{i}^{T} \mathbf{h}_{j} - \sum_{n=1}^{N_G} 
    %\mathbb{E}_{v_n \sim P_{G}(v)} 
    \mathbf{h}_{i}^{T} \mathbf{h}_{n} \right), 
\end{aligned}
\end{equation}
where $\mathbf{h}_i$ is the learned embedding for road $v_i$, $N_G$ is the predefined negative size for \textit{graph reconstruction} task, and $v_n$ is the negative road segment sampled by $v_n \sim P_{G}(v)$. We will discuss the implementation of $P_{G}(v)$ in the following section.

\textbf{Hypergraph-level Pretext Task.} Based on the proposed hypergraph structure, we design two new self supervised learning tasks, \textit{hypergraph reconstruction} and \textit{hyperedge classification}, to inject prior knowledge and provide useful signals to guide road representation learning.

\begin{itemize}[leftmargin=*]
  \item \textit{Hypergraph Reconstruction.} Intuitively, the node and its hyperedge context should share similar representations. For example, the road segments in a highway ring tend to serve similar functions. Thus, we propose to preserve this kind of correlations by reconstructing the incidence matrix $\mathbf{H}$ in $\mathcal{G_H}$. Similarly, the objective function can be formulated as follows.
  
\begin{equation}
\begin{aligned}
    \mathcal{L}_{HR} = - \sum_{v_i \in \mathcal{V}} \sum_{e_j \in \mathcal{H}_i} \left(\mathbf{h}_{i}^{T} \mathbf{m}_{j} - \sum_{n=1}^{N_H} \mathbf{h}_{i}^{T} \mathbf{m}_{n} \right), 
\end{aligned}
\end{equation}

where $\mathbf{m}_j$ is the learned embedding for hyperedge $e_j$ in the last layer, $\mathcal{H}_i$ represents the neighbor hyperedge set of node $v_i$ such that $\mathbf{H}_{i,j} = 1$, and $N_H$ denotes the predefined negative size for \textit{hypergraph reconstruction} task. For each positive pair $(v_i, e_j)$, we fix road $v_i$ and sample other hyperedge $e_n \sim P_{H}(e)$ as negative pairs. 
  
\item \textit{Hyperedge classification.} To deal with the long range correlation issue, we inject the prior knowledge named hyperedge cluster relationships into training tasks. As discussed in Section \ref{sec:intro} and \ref{sec:pf}, the cluster of hyperedge can serve as a medium to capture road correlations through 'road-hyperedge-cluter-hyperedge-road' scheme. Specifically, given a hyperedge $e_i$ and its representation $\textbf{m}_i$, we aim at predicting the cluster label $c_i$ based on the learned representation. Formally, we define a classification pretext task by adopting the categorical cross-entropy loss function as follows. 

\begin{equation}
\begin{aligned}
    \mathcal{L}_{HC} = - \sum_{e_i \in \mathcal{E_H}} \left(\sum_{k=1}^{K} \log \frac{\exp(x_{i,k})}{\sum_{k^\prime} \exp(x_{i,k^\prime})} \cdot y_{i,k} \right), 
\end{aligned}
\end{equation}

where $K$ is the number of clusters, $y_{i,k}$ is set to 1 when $k=c_i$ and 0 for other cases, $x_{i,k}$ is the $k$-th dimension of output vector $\mathbf{x}_i$ obtained by transforming hyperedge representation $\mathbf{m}_i$ as $\mathbf{x}_i = \text{MLP}(\mathbf{m}_i)$. 
\end{itemize}

Finally, we unify the different pretext tasks into a multi-task learning framework. The joint learning objective function is as follows, where $\alpha$ is hyper-parameter controlling the contributions from graph-level and hypergraph-level pre-training.

\begin{equation}
\mathcal{L} = \mathcal{L}_{GR} + \alpha \cdot (\mathcal{L}_{HR} + \mathcal{L}_{HC}).
\end{equation}


\textbf{Discussion on Negative Sampling.} Recall that we introduce two negative sampling distributions $P_G(v)$ and $P_H(e)$ in graph-level and hypergraph-level pretext task respectively. In this section, we provide two implementations for this framework named \textit{random sampling} and \textit{distance based sampling}.

\begin{itemize}[leftmargin=*]
\item \textit{Random Sampling.} One natural way is to perform uniform sampling. Specifically, given a context node $v_i$, we uniformly sample nodes from outside its neighborhoods $\mathcal{N}_i$, and set the probability of a candidate node $v_n$ as 
%$P_G(v_n|v_i) = 1/|\mathcal{V} \backslash \mathcal{N}_i|$.
$P_G(v_n|v_i) = \frac{1}{|\mathcal{V} \backslash \mathcal{N}_i|}$.
Similarly, we sample negative hyperedges from outside $v_i$'s neighborhoods $\mathcal{H}_i$ in hypergraph, and define the distribution as 
%$P_H(e_n|v_i) = 1/|\mathcal{E_H} \backslash \mathcal{H}_i|$.
$P_H(e_n|v_i) = \frac{1}{|\mathcal{E_H} \backslash \mathcal{H}_i|}$.

\item \textit{Distance Based Sampling (DBS for short).} Motivated by Tobler’s First Law of Geography \cite{miller2004tobler}, which states that everything is related to everything else, but near things are more related than distant things, we propose another negative sampling method based on distance. Given a context node $v_i$, we calculate the pairwise distance between it and all other nodes using shortest path distance. Formally, we define $D_G(v_i, v_n)$ to denote the distance between $v_i$ and $v_n$. Then, the probability of node $v_n$ ($v_n \notin \mathcal{N}_i$) being a negative sample is given as follows.

\begin{equation}
P_G(v_n|v_i) = \frac{D_G(v_i, v_n)}{\sum_{v_{n^\prime} \in \mathcal{V} \backslash \mathcal{N}_i} D_G(v_i, v_{n^\prime})}.
\end{equation}

In general, the larger the distance, the more likely the node $v_n$ is sampled as a negative sample for context $v_i$. Following a similar idea, we first define the distance between node $v_i$ and hyperedge $e_n$ as:

\begin{equation}
D_H(v_i, e_n)=\frac{1}{|\mathcal{R}_n|}\sum_{v_j \in \mathcal{R}_n} D_G(v_i, v_j),
\end{equation}

where $D_H(v_i, e_n)$ is the average of multiple  node pair distances, $\mathcal{R}_n$ denotes the set of nodes connected to hyperedge $e_n$ in $\mathcal{G_H}$. Then, the sampling probability of negative hyperedge $e_n$ ($e_n \notin \mathcal{H}_i$) can be give in a similar way as:

\begin{equation}
P_H(e_n|v_i) = \frac{D_H(v_i, e_n)}{\sum_{e_{n^\prime} \in \mathcal{E_H} \backslash \mathcal{H}_i} D_H(v_i, e_{n^\prime})}.
\end{equation}

\end{itemize}

Considering the high time and space complexity of distance calculation, we use \textit{random sampling} as the default choice in HyperRoad and empirically compare different sampling methods in Section \ref{sec:q2}. 


==> inputs/problem_formulation.tex <==
\section{Problem Statement} \label{sec:pf}
In this section, we present the notations and several preliminaries first and then define our problem formally.

\textbf{Definition 1. Road Network:} A road network is represented as a directed graph $\mathcal{G_R}=(\mathcal{V}, \mathcal{E_R}, \mathcal{P})$, where $\mathcal{V} = \{v_1, v_2, \dots, v_N\}$ is a set of nodes (i.e., road segments) \footnote{We use node and road segment interchangeably in this paper.}, $\mathcal{E_R}$ is a set of edges and its corresponding adjacency matrix is represented as $\mathbf{A} \in \mathbb{R}^{N \times N}$. Each entry $\mathbf{A}_{i,j}$ is a binary value indicating whether there exists a link between road segment $v_i$ and road segment $v_j$. Each node $v_i$ has a coordinates vector $\mathbf{p}_i$ including latitude and longitude, mapping the road segment into geographic space. 

\textbf{Definition 2. Hypergraph:} Different from simple graph, a hypergraph is a more general topological structure where a hyperedge could connect two or more nodes. A hypergraph based on road network is defined as $\mathcal{G_H}=(\mathcal{V}, \mathcal{E_H})$, where $\mathcal{V}$ is a set of road segments shared with road network $\mathcal{G_R}$, and  $\mathcal{E_H} = \{e_1, e_2, ... , e_M\}$ represents the set of hyperedges. Notably, the topological structure of $\mathcal{G_H}$ can also be represented by an incidence matrix $\mathbf{H} \in \mathbb{R}^{N \times M}$, with entries defined as:

\begin{equation}
\label{eq:hg}
\mathbf{H}_{i,j} = \left\{
    \begin{aligned}
        1 & , & \text{if} \,\, v_i \in e_j, \\
        0 & , & \text{if} \,\, v_i \notin e_j.
    \end{aligned} \right.
\end{equation}

In order to model high-order road segment relations, we construct hyperedges on road network as follows.  

\textbf{Hypergraph construction strategy in road network.} As can be seen in Fig. \ref{fig:intro}, the surround structure in the road network (like a polygon indicated by blue dotted frame in Fig. \ref{fig:intro}) has rich semantic information and physical meaning. On one hand, it preserves node homogeneity in a long range mostly. For example, the road segments in the polygon tend to be similar road types. On the other hand, it introduces inductive bias for road network modelling. For example, a building is more likely to be surrounded by a small number of residential road segments and form a relatively small polygon (two blue dotted frames in Fig. \ref{fig:intro} surround a few road segment with residential functions and thus semantic dependencies are constructed despite they are far apart). While a hill is more likely to be surrounded by many motorways and result in a large polygon (considering the red road segments in Fig. \ref{fig:intro}). To leverage the inductive bias and prior domain knowledge, we construct hypergraphs based on this special structure firstly. Specifically, we apply map segmentation algorithm proposed in \cite{yuan2012discovering} to split the road network into different polygons, and consider each one as a hyperedge and it will connect all the road segments within this small area. Then, the incidence matrix $\mathbf{H}$ for hypergraph can be constructed based on the above results. We further cluster each polygon (\textit{e.g.}, hyperedge) into $K$ different clusters based on its features including area and number of sides. Formally, we reformulate the hypergraph as $\mathcal{G_H}=(\mathcal{V}, \mathcal{E_H}, \mathcal{C})$ where each hyperedge $e_i \in \mathcal{E_H}$ is assigned to a cluster label $c_i \in \mathcal{C}$. 

% It is worth mentioning that although we only discuss the surround structure based hyperedges in this study, other meaningful hyperedges can also be integrated into the proposed model to further improve road segment representation learning. For example, the trajectory is a special kind of hyperedge which captures complex human moving behaviors on road network. However, it may suffer from coverage and availability problems. We leave this aspect to future works.


\textbf{Problem Statement:} Given a road network $\mathcal{G_R}=(\mathcal{V}, \mathcal{E_R}, \mathcal{P})$, and a hypergraph $\mathcal{G_H}=(\mathcal{V}, \mathcal{E_H}, \mathcal{C})$ built on $\mathcal{G_R}$, we aim to learn a low dimensional vector representation for each road segment, which can be denoted as $\{\mathbf{h}_i | \mathbf{h}_i \in \mathbb{R}^{d} \}_{v_i \in \mathcal{V}}$ with $d$ as the embedding size. 

==> inputs/related_work.tex <==
\section{Related Work}\label{sec:relate}
Our work is related to the following topics including graph representation learning, road networks modelling and hypergraph learning.  

\subsection{Graph Representation Learning}
Recent years have witnessed the great success of representation learning in modelling graph data. %\cite{goyal2018graph}. 
The earliest efforts in this field mainly focus on shallow representations. For example, DeepWalk \cite{perozzi2014deepwalk} and Node2Vec \cite{grover2016node2vec} use random walks on the graph to generate node sequence and then apply skip-gram model \cite{mikolov2013distributed} to learn node representations. LINE \cite{tang2015line} aims to preserve first and second-order proximity by explicitly modelling the corresponding objectives. And all these models are actually equivalent to the simple matrix factorization framework with closed forms \cite{qiu2018network}.  Inspired by the recent huge success of deep learning, neural networks have also been introduced for graph representation learning. Along this line, graph convolution networks (GCN) \cite{kipf2016semi} and graph attention network (GAT) \cite{velivckovic2017graph} are two classic models. These GNN models mainly follows the paradigm of message passing and local neighborhood aggregation. Based on such a core architecture, different 
variants are proposed by exploring various aggregation operations \cite{xu2018powerful, hamilton2017inductive}. 

However, all these methods are not designed for road networks and fail to capture unique structure information in road networks such as the long range road segment correlations.
% need to detail in the introduction section.

\subsection{Road Networks Modelling} As the basic component of the transportation systems, road network has been used to facilitate various transportation applications, such as traffic inference and forecasting \cite{hu2019stochastic, guo2019attention}, as well as road tags prediction \cite{yin2021multimodal}.
%and region functionality modelling \cite{wozniak2021hex2vec}. 
In these methods, road segment embedding are indirectly learned as a byproduct to incorporate spatial and graph topology information. For example, A-GCWC \cite{hu2019stochastic} employs graph convolution network to impute road traffic speed and road embedding is correspondingly generated as a byproduct of input module. However, these methods are tailored for specific tasks which are difficult to transfer to other problems. Recently, a few studies propose to learn generic road embeddings by extending graph representation learning to road networks \cite{jepsen2020relational, wang2019learning, wu2020learning, chen2021robust}. In specific, IRN2Vec \cite{wang2019learning} extends DeepWalk by considering geo-locality and geo-shape information, while HRNR \cite{wu2020learning} extend GCN by considering hierarchical structures. 

However, none of these methods propose to learn high-order road segment interactions, which is vital for high-quality representation learning. They suffer from either shallow representation or expressive power issues. Meanwhile, these approaches focus on local neighborhoods and thus 
fail to thoroughly address the long range correlation problem. 

\subsection{Hypergraph Learning}
Hypergraph learning is firstly introduced in \cite{zhou2006learning} to generalizing the methodology of spectral clustering to hypergraphs, which naturally models high-order relations of three or more entities. The subsequent works also adopt ranking based methods \cite{li2013link} and non-negative matrix factorization methods \cite{zhang2018beyond} for hypergraph mining and hyperedge prediction. Until very recently, deep learning based methods have been developed in this field. In specific, deep neural networks and auto-encoder are applied in DHNE \cite{tu2018structural} to capture first-order proximity and second-order proximity respectively for hyperedge representation learning. Zhang et al. \cite{zhang2019hyper} applied attention mechanism and MLP network for both dynamic and static hyperedge representations learning and thus improve hyperedge prediction performance. Recently, hypergraph neural networks (HGNNs) \cite{feng2019hypergraph}
%\cite{feng2019hypergraph, jiang2019dynamic} 
have been further proposed to generalize the neighborhood aggregation operation to the hypergraph. 

However, to our best knowledge, our proposed method is the first attempt to shift the power of hypergraph to the road network modeling. We design meaningful hypergraph construction strategy in road network for the first time, and then propose hypergraph based dual-channel aggregation mechanism and self supervised learning tasks for effective representation learning, which compose the key contributions.

==> inputs/response.tex <==
\clearpage
\newpage
% \balance
\noindent{\normalsize \textbf{Response Letter for Submission TKDD-2022-11-0442 ``Road Network Representation Learning: Hypergraph is Also
What You Need''}}

\noindent
We would like to sincerely thank the reviewers and associate editor for their valuable comments and suggestions. We have revised our paper accordingly. Below please find our detailed responses to the reviewers' comments (denoted by ``D''). 

\section*{Associate Editor}
\centerline{\textbf{Comment D0.1}}
\noindent\emph{\textcolor{blue}{The reviewers have raised concerns around novelty of the method, and also contextualizing of the paper in the realm of related work. I hope you find the reviewers' comments helpful in improving the paper.}}

\noindent\textbf{Response A0.1:}
Thanks for giving us the opportunity to revise this paper. Upon the reviewers’ constructive comments, we revised the manuscript in the following aspects:

\begin{itemize}[leftmargin=*]
    \item We have elaborated more on the motivations of the proposed model and discussed the rationale
    {\chengr behind the modules of the model.}
    % of different modeling modules.
    \item We have conducted more ablation studies to better validate the effectiveness and novelty of our module design.
    \item We have provided detailed descriptions of the experimental setup and more discussion on the experiment results. 
    \item We have referred to more related work of this paper and  thoroughly edited the paper to improve the readability. 
\end{itemize}

The responses to the reviewers' comments are detailed as follows.

\vspace*{1\baselineskip}
\section*{Reviewer 1}

\centerline{\textbf{Comment D1.1}}
\noindent\emph{\textcolor{blue}{In the title, the phrase “Hypergraph is also what you need” sounds awkward. I understand the reference to the “Attention is all you need” paper and the authors’ combining a simple graph and hypergraph representation, but it doesn’t really make sense grammatically, and could mislead readers into thinking the paper is about attention mechanisms.}}\\
\noindent\textbf{Response A1.1:} 
% Thank you very much for your careful checking and comments. We are not sure if it is possible to change the title during the revision process. However, if the paper could be accepted, we would change the title to ``Road Network Representation Learning: A Dual Graph Perspective'' following your advice. 
{\chengr Thank you very much for your comments. We shall check with the Editor-in-Chief and see if it would be possible to update the title. If so, we plan to update the title to be ``Road Network Representation Learning: A Dual Graph based Approach''.}
\vspace*{1\baselineskip} 

\centerline{\textbf{Comment D1.2}}
\noindent\emph{\textcolor{blue}{Section 6.3: could the authors please confirm that alpha is the same alpha used in Eq. 12 to weight the reconstruction term in the loss function?}}\\
\noindent\textbf{Response A1.2:}  
% We use the same alpha to weight the reconstruction term in loss function Equation~\eqref{eq:loss_base} since the last two pretext tasks (hypergraph reconstruction and hyperedge classification) are both hypergraph-level.
{\chengr We use the same alpha to weight the losses of the last two pretext tasks (hypergraph reconstruction and hyperedge classification) in Equation~\eqref{eq:loss_base} since they are both hypergraph-level tasks.}
\vspace*{1\baselineskip}

\centerline{\textbf{Comment D1.3}}
\noindent\emph{\textcolor{blue}{Pg 3, line 51: I think this sentence should read “hypergraph reconstruction and hyperedge classification.”}}\\
\noindent\textbf{Response A1.3:} Thanks for pointing it out. We have revised {\chengr the sentence} accordingly.
\vspace*{1\baselineskip}

\centerline{\textbf{Comment D1.4}}
\noindent\emph{\textcolor{blue}{While I think the paper is strong in its application to road networks, the key methodological contributions of the proposed lack some novelty and conversation with important recent works on graph neural networks. Specifically, Several recent works, such as Chen et al. [1], have already utilized residual connections to facilitate learning long-range dependencies in graphs.}}\\
\noindent\textbf{Response A1.4:} 
{\chengr We} have added the discussion {\chengr on the} reference (Chen et al. [1]) to {\chengr the methodology part} (Section \ref{sec:fusion}, line 263-266). {\chengr Specifically,} most GNN methods capture the long-range dependencies in graphs by broadening the receptive fields in message propagation. {\chengr Some existing studies such as} Chen et al. [1] utilize residual connections to alleviate the over-smoothing problem when building deep graph neural networks. The residual connections used in our paper serve similar functions. 

% However, since our target is road network, the intrinsic properties associated with the road network can be used as inductive bias to help capture the long-range dependencies from another perspective apart from stacking deep graph neural networks. Specifically, as can be seen from Fig \ref{fig:revision_case}, ``Road B'' and ``Road C'' serve as similar urban functions (e.g., they are both residential roads with low speed limit) despite being far apart on the map, and thus they establish a kind of typical long-range dependency in the road network. The so-called urban functions can be partly reflected by the behaviors of how roads form local regions in the real world. For example, the residential roads tend to form smaller area indicated by the blue dotted frames while the highway roads tend to form a larger region as indicated by the red highway loop. Therefore, by clustering the hyperedges ({\it{i.e.}}, local regions) using the prior knowledge and proposing the hyperedge classification pretext task, ``Road B'' and ``Road C'' can have similar representations since they belong to the same hyperedge cluster where hyperedges serve as ``bridges''.  

% \begin{figure}[h]
% 	\centering
% 	\includegraphics[width=0.50\textwidth]{inputs/Figs/intro_case.pdf}
% 	\caption{Road network example.}
% 	\label{fig:revision_case}
% 	\vspace{-0.1cm}
% \end{figure}

\vspace*{1\baselineskip}

\noindent{[1]. Chen, Ming, et al. "Simple and deep graph convolutional networks." International conference on machine learning. PMLR, 2020.}
\vspace*{1\baselineskip}

\centerline{\textbf{Comment D1.5}}
\noindent\emph{\textcolor{blue}{The inclusion of a self-supervised reconstruction term in the loss function is common in graph autoencoders, and has also been proposed for hypergraph autoencoders [2]. The authors mention this briefly in Section 7 (e.g. in relation to Tu et al., 2018), but given that the authors claim this as a key methodological contribution, more comparison is needed -- especially in Section 3.3.}}\\
\noindent\textbf{Response A1.5:} 
We design two types of pretext tasks for RNRL, namely graph-level and hypergraph-level tasks, to effectively encode the road network structures into representations. The graph-level tasks refer to graph reconstruction, while the hypergraph-level tasks refer to hypergraph reconstruction and hyperedge classification. Among them, the graph reconstruction pretext task {\chengr has already been} applied in some existing RNRL models \cite{jepsen2020relational, wu2020learning} and the hypergraph reconstruction task is natural for hypergraph representation learning such as hypergraph auto-encoder \cite{wang2016structural, hu2021adaptive}. 
{\chengr We emphasize that} our self supervised learning component differs from existing methods in (1) it introduces the hypergraph reconstruction task in road network representation learning problem for the first time; and (2) it combines both graph-level tasks and hypergraph-level tasks in a unified framework for the first time; and (3) it proposes a new pretext task named hyperedge classification for the constructed hyperedges based on prior knowledge of road networks.
{\chengr We have included this} discussion as well as references {\chengr in the methodology part} (Section \ref{sec:ssl}, line 280-289).

{\chengr In addition,} we verify the above discussion with experimental results. Apart from w/o GPT where the graph-level tasks are removed and w/o HPT where hypergraph-level tasks are removed entirely, we propose another model variant here named w/o HEC where only hyperedge classification task is removed. The ablation study results are shown in Table \ref{tab:hec_task}. From the results, we {\chengr have} the following observations. 1) w/o HPT applies graph reconstruction task while w/o HEC applies both graph and hypergraph reconstruction tasks. By comparing these two methods, we can find that introducing hypergraph reconstruction task in road network representation learning indeed brings advantages in Road Type prediction application, which support the first discussion ({\textbf{it introduces the hypergraph reconstruction task in road network representation learning problem for the first time}}). However, simply combing two commonly used reconstruction tasks also brings noise for some other downstream applications. 2) HyperRoad which considers both graph-level and hypergraph-level tasks outperforms w/o GPT and w/o HPT. The results support the second discussion ({\textbf{it combines both graph-level tasks and hypergraph-level tasks in a unified framework for the first time}}). 3) HyperRoad achieves significant improvements compared with w/o HEC, showing the importance of the proposed hyperedge classification task. It supports the last discussion ({\textbf{it proposes a new pretext task named hyperedge classification for the constructed hyperedges based on prior knowledge of road networks}}). 

{\chengr We have included the above} experiment results {\chengr to the Ablation Study (RQ2) part} (Section \ref{sec:q2}, line 532-534, 558-572).

\begin{table*}[h]
	\renewcommand{\arraystretch}{1.15} 
	\centering 
	\caption{Ablation studies for self-supervised learning on Singapore dataset.}
    \normalsize
	\resizebox{0.99\linewidth}{!}{
		\begin{tabular}{c|ccc|ccc|ccc|ccc}
			\toprule
			\multirow{3}{*}{Model} & \multicolumn{3}{c|}{{\textbf{ One/Two Way}}} & \multicolumn{3}{c|}{{\textbf{No. of Lanes}}} & \multicolumn{3}{c|}{{\textbf{Speed Limit}}} & \multicolumn{3}{c}{{\textbf{Road Type}}} \\
			\cmidrule{2-13}
			& Micro-F1 & Macro-F1 & Weighted-F1 & Micro-F1 & Macro-F1 & Weighted-F1 & Micro-F1 & Macro-F1 & Weighted-F1 & Micro-F1 & Macro-F1 & Weighted-F1  \\ \midrule
			w/o GPT  & \underline{0.7804} & \underline{0.6875} & \underline{0.7593} & 0.4793 & 0.1403 & 0.3293 & 0.5876 & 0.1952 & 0.4568 & \underline{0.5742} & \underline{0.3466} & \underline{0.5316}\\
			w/o HPT & 0.7402 & 0.5965 & 0.6980 & \underline{0.4827} & \underline{0.1465} & \underline{0.3327} & \underline{0.6016} & \underline{0.2341} & \underline{0.4885} & 0.5220 & 0.3598 & 0.4937\\
            w/o HEC & 0.7239 & 0.5442 & 0.6648 & 0.4794 & 0.1287 & 0.3243 & 0.5945 & 0.1602 & 0.4572 & 0.5553 & 0.3679 & 0.5217 \\
		    \midrule
			HyperRoad & \textbf{0.7864} & \textbf{0.6995} & \textbf{0.7676} & \textbf{0.4829} & \textbf{0.1534} & \textbf{0.3392} & \textbf{0.6066} & \textbf{0.2534} & \textbf{0.4970} & \textbf{0.5785} & \textbf{0.3964} & \textbf{0.5482}\\ 
			\bottomrule
	\end{tabular}}
	\label{tab:hec_task}
\vspace{-0.1cm}
\end{table*}

\vspace*{1\baselineskip}

\noindent{[2] Hu, Youpeng, Xunkai Li, Yujie Wang, Yixuan Wu, Yining Zhao, Chenggang Yan, Jian Yin, and Yue Gao. "Adaptive hypergraph auto-encoder for relational data clustering." IEEE Transactions on Knowledge and Data Engineering (2021).}
\vspace*{1\baselineskip}


\centerline{\textbf{Comment D1.6}}
\noindent\emph{\textcolor{blue}{The dual-channel aggregation mechanism, which the authors use to learn representations from both the simple graph and hypergraph, is not that different from other works on higher-order graph neural networks, such as Morris et al. [3]. The proposed work does differ in that it uses two different representations (simple graph and hypergraph) rather than learning representations for k-order cliques on the same graph as in Morris et al. I'm not aware of other works that use both a simple graph and a hypergraph together, so I think this is an interesting contribution, but the similarity to higher-order GNNs should at least be mentioned.}}\\
\noindent\textbf{Response A1.6:} 
% Thanks for your kind advice. 
We have added some discussion {\chengr on the difference between our model and existing higher-order GNNs} to the methodology {\chengr part} (Section \ref{sec:dual-channel}, line 230-238). 
% We copy the discussion here for a quick reference. 
Specifically, some existing GNN methods \cite{morris2019weisfeiler, wang2021tree} also model high-order node relationships to help expand the receptive fields and/or improve the expressiveness of GNN model. For example, $k$-GNNs \cite{morris2019weisfeiler} aggregates the information from high-order neighbors defined by the $k$-order cliques, and TDGNN \cite{wang2021tree} aggregates the information from multi-hop neighbors defined by the tree decomposed subgraphs. These methods define different structures on the same simple graph. {\chengr In contrast}, our aggregation mechanism {\chengr takes} a dual graph perspective and aggregates information from both simple graph and hypergraph. In fact, we are aware of no existing methods which use multiple channels to combine a simple graph and a hypergraph together as ours does.

We also verify the {\chengr above} discussion with experimental results. Previously, we have compared with the model variant w/o DAM where we only use the hyperedge channel aggregation to update the road representations ({\emph{i.e.}}, w/o DAM (HGNN)). {\chengr We further add an} ablation study about the aggregation mechanism. Specifically, we replace the dual channel aggregation with the k-GNN component proposed in \cite{morris2019weisfeiler} ([3]) and name this base model as AM-KGNN. The experiment results are presented in Table \ref{tab:agg_mec}. From the results, we have the following findings. 

1) AM-KGNN mainly aggregates information from the simple graph channel (% it defines different 
{\chengr note that the $k$-order cliques defined by AM-KGNN are all} based on the same simple graph), and w/o DAM aggregates information from the other hypergraph channel. We can find that AM-KGNN performs better on One/Two Way prediction while w/o DAM performs better on Speed Limit prediction application.
% showing that {\chengr using only a} single graph aggregation {\chengr channel} is not enough. 
%
2) HyperRoad applies two separate channels to capture different graph structure information in both simple graph and hypergraph and thus it outperforms AM-KGNN on all {\chengr tasks}. The results demonstrate the novelty and importance of our proposed dual-channel aggregation mechanism and it cannot be simply replaced with existing GNN components. 

{\chengr We have included the above} experiment results to the Ablation Study (RQ2) part (Section \ref{sec:q2}, line 525-528, 551-554).

\begin{table*}[h]
	\renewcommand{\arraystretch}{1.15} 
	\centering 
	\caption{Ablation studies for aggregation mechanism.}
    \normalsize
	\resizebox{0.99\linewidth}{!}{
		\begin{tabular}{c|ccc|ccc|ccc|ccc}
			\toprule
			\multirow{3}{*}{Model} & \multicolumn{3}{c|}{{\textbf{ One/Two Way}}} & \multicolumn{3}{c|}{{\textbf{No. of Lanes}}} & \multicolumn{3}{c|}{{\textbf{Speed Limit}}} & \multicolumn{3}{c}{{\textbf{Road Type}}} \\
			\cmidrule{2-13}
			& Micro-F1 & Macro-F1 & Weighted-F1 & Micro-F1 & Macro-F1 & Weighted-F1 & Micro-F1 & Macro-F1 & Weighted-F1 & Micro-F1 & Macro-F1 & Weighted-F1  \\ \midrule
            w/o DAM (HGNN) & 0.7545 & 0.6221 & 0.7164 & \underline{0.4784} & \underline{0.1183} & 0.3145 & \underline{0.5929} & \underline{0.1928} & \underline{0.4544} & 0.5497 & \underline{0.3609} & 0.5114 \\ 
			AM-KGNN & \underline{0.7832} & \underline{0.6903} & \underline{0.7618} & 0.4768 & 0.1174 & \underline{0.3148} & 0.5897 & 0.1555 & 0.4447 & \underline{0.5587} & 0.3022 & \underline{0.5120} \\
		    \midrule
			HyperRoad & \textbf{0.7864} & \textbf{0.6995} & \textbf{0.7676} & \textbf{0.4829} & \textbf{0.1534} & \textbf{0.3392} & \textbf{0.6066} & \textbf{0.2534} & \textbf{0.4970} & \textbf{0.5785} & \textbf{0.3964} & \textbf{0.5482}\\ 
			\bottomrule
	\end{tabular}}
	\label{tab:agg_mec}
\vspace{-0.1cm}
\end{table*}

\vspace*{1\baselineskip}

\noindent{[3] Morris, Christopher, Martin Ritzert, Matthias Fey, William L. Hamilton, Jan Eric Lenssen, Gaurav Rattan, and Martin Grohe. "Weisfeiler and leman go neural: Higher-order graph neural networks." In Proceedings of the AAAI conference on artificial intelligence, vol. 33, no. 01, pp. 4602-4609. 2019.}
\vspace*{1\baselineskip}

\centerline{\textbf{Comment D1.7}}
\noindent\emph{\textcolor{blue}{First, the discussion about long-range dependencies is extremely unconvincing. In addition to the related work I mentioned above, I see no reason why a hypergraph can model these dependencies better than a simple graph. The authors state that the hyperedges serve as ``bridges,'' but this claim is not justified anywhere in the text or any related work, and there is nothing in Eqs 4-7 that solve this problem any better than a message-passing GNN on a simple graph. My honest recommendation to the authors would be to remove the discussion of long-range dependencies entirely from the paper.}}\\ 
% To do
\noindent\textbf{Response A1.7:} 
% Sorry for the misleading description in our paper. In fact, we are not claiming that the aggregation mechanism described by Equations (\ref{eq:4}) - (\ref{eq:7}) can model these dependencies better than a message-passing GNN on a simple graph. As discussed in our response \textbf{A1.4}, we capture one of the most typical long-range dependencies in road network through the proposed hyperedge classification pretext task in Equation (\ref{eq:loss_base}), where two remote roads can share information since they belong to the same hyperedge cluster and the hyperedges serve as ``bridges'' here. The behind motivation is the physical logic of road network construction, which is special for road network and differs from other general graphs. We also verify the advantages of introducing such dependencies via experiments shown in our \textbf{response A1.5} (or Table \ref{tab:hec_task}). 
% However, since our target is road network, the intrinsic properties associated with the road network can be used as inductive bias to help capture the long-range dependencies from another perspective apart from stacking deep graph neural networks. 
{\chengr First of all, we clarify the meaning of ``long-range relationships''. They refer to cases where two roads that are can be far from each other share some semantics. For example, in Fig. \ref{fig:intro},} 
% Specifically, as can be seen from Fig \ref{fig:intro}, 
``Road B'' and ``Road C'' serve similar urban functions (e.g., they are both residential roads with low speed limit) despite being far apart on the map.
% , and thus they establish a kind of typical long-range dependency in the road network. 
% The so-called urban functions can be partly reflected by the behaviors of how roads form local regions in the real world. For example, the residential roads tend to form smaller area indicated by the blue dotted frames while the highway roads tend to form a larger region as indicated by the red highway loop. Therefore, by clustering the hyperedges ({\it{i.e.}}, local regions) using the prior knowledge and proposing the hyperedge classification pretext task, ``Road B'' and ``Road C'' can have similar representations since they belong to the same hyperedge cluster where hyperedges serve as ``bridges''.   
{\chengr Second, our saying that ``hyperedges serve as bridges for capturing long-range relationshps'' can be misleading. It does not mean that we capture the long-range relationships via message propagation along hyperedges (as formalized in Eqs 4-7). In fact, we capture the long-range relationships mainly with the hyperedge classification pretext task. Specifically, we cluster the hyperedges based on hyperedges' properties such as sizes and use the cluster IDs as the class labels for the hyperedge classification task. The hyperedges' labels act as a medium to share information among roads that may be far apart through a ``road-hyperedge-cluster-hyperedge-road'' scheme for capturing long-range relationships. For example, ``Road B'' and ``Road C'' in Fig. \ref{fig:intro} are involved in hyperedges with similar sizes (which tend to have similar urban functions and belong to the same hyperedge cluster), and thus they would tend to have similar representations.
}
% \begin{figure}[h]
% 	\centering
% 	\includegraphics[width=0.50\textwidth]{inputs/Figs/intro_case.pdf}
% 	\caption{Road network example.}
% 	\label{fig:revision_case}
% 	\vspace{-0.1cm}
% \end{figure}

\textbf{In summary}, the aggregation mechanism described by Equations (\ref{eq:4}) - (\ref{eq:7}) performs information propagation in both simple graph and hypergraph structures, and thus it naturally captures pairwise relationships and high-order relationships among the roads. Meanwhile, the hyperedge classification pretext task (in bi-level self supervised learning) described by Equations (\ref{eq:loss_base}) incorporates domain knowledge and helps to capture the long-range relationships in road network. Finally, combining these components in a unified framework, our proposed method is capable of modeling the pairwise, high-order and long-range relationships among the roads all at the same time. 

We have carefully revised all relevant descriptions of our paper in Abstract (line 15-17), Introduction (Section \ref{sec:intro}, line 85-90, 98-99, 127-133) as well as Methodology (Section \ref{sec:HC}, line 212-217, 311-320) to {\chengr reflect the above discussions on long-range relationships and how we capture them.}

\vspace*{1\baselineskip}

\centerline{\textbf{Comment D1.8}}
\noindent\emph{\textcolor{blue}{As a further point, Figs 3 and 5 are also very unconvincing. Long-range and higher-order dependencies, as typically discussed in the literature, are very different than simple correlations between features of sampled edges. I also don't think these figures are necessary; the existence of these dependencies in graphs is well established and also demonstrated by the authors experimental results.}}\\
\noindent\textbf{Response A1.8:} Thanks for your advice. We have removed the corresponding figures as well as associated descriptions in our paper.
\vspace*{1\baselineskip}

\centerline{\textbf{Comment D1.9}}
\noindent\emph{\textcolor{blue}{Second, section 5 needs more detail on the training/testing setup. At minimum, readers need to know how the data set was divided into training and testing sets, and how the final results were computed. Were there multiple testing folds (i.e., cross validation)? If there was only a single testing fold, at minimum the authors should report the results from multiple iterations of the experiments, along with standard deviations, since neural networks can be sensitive to both distribution shift (from training to test set) and the random parameter initialization.}}\\
\noindent\textbf{Response A1.9:} 
% Thank you very much for your careful checking and we are sorry for missing this part. 
{\chengr Thank you for the comments. We should have provided these details of experimental set-up.}
For training/testing setup, we apply 5-fold cross validation to evaluate the performance of all the methods. We have added {\chengr these} details to our experimental setup (Section \ref{sec:dataset}, line 467-471). We copy the descriptions here for a quick reference. Specifically, for all the mentioned tasks, we apply 5-fold cross validation to evaluate the performance of all the methods. For example, for the road based tasks, we use 4-fold road representations and their tag labels as training data and {\chengr use} the rest 1-fold data as test set (we also randomly sample 10\% of each training fold to act as a validation set during training process). {\chengr We report the average of} the results of 5-fold test sets.
\vspace*{1\baselineskip}

\centerline{\textbf{Comment D1.10}}
\noindent\emph{\textcolor{blue}{While less significant, a concern I have about the results: in Table 1, why is macro F1 so much lower than micro F1 in several cases? This makes me concerned that either there is something strange in the experimental setup or that there is a significant bias toward the majority class(es) in model predictions. The authors should address this difference.}}\\
\noindent\textbf{Response A1.10:} 
% Since our target is road network, 
{\chengr The main reason is that}
the tags for road network are unevenly distributed in the real world. For example,  most roads have 2 lanes and very few roads have 5 lanes. Analogously, most roads have a maximum speed limit of 50 (or 40), while a few roads have a maximum speed limit of 70 and 80. Therefore, the model predictions are indeed biased towards the majority class(es) in some cases and lead to small macro-F1 scores. 
%
% However, as can be seen from Table \ref{tab:classify} and Table \ref{tab:A_T_AT}, 
{\chengr We emphasize that} our model outperforms existing methods not only in terms of micro-F1 (which means our model achieves better overall accuracy), but also in terms of macro-F1 (which means our model is less biased towards the majority class(es)). The underlying reason is that our model can better distinguish roads with different semantics, as shown in Fig. \ref{fig:embedding}, and thus it {\chengr can} predict road labels even for roads belonging to small class(es).

\vspace*{1\baselineskip}

\centerline{\textbf{Comment D1.11}}
\noindent\emph{\textcolor{blue}{One more (relatively minor) comment: It’s strange to me that GraphSAGE outperforms the application-specific baselines in several cases. For example, in the HRNR paper, HRNR outperforms GAT, which I would expect to outperform GraphSAGE in the road network setting. This might not be a particularly important point, but stood out to me as a reviewer.}}\\
\noindent\textbf{Response A1.11:} 
% Since we identify four settings for RNRL depending on the availability of the road attributes and trajectories for the first time, we propose to use different names for baselines with different versions. 
{\chengr This is because in the original HRNR paper, the model consider all types of information including spatial and structural information, attributes, and trajectory data as input. We name this model as ``HRNR-AT'' in our paper. In contrast, HRNR in our paper corresponds to ``HRNR-AT'' (the model in the original HRNR paper) by dropping the components for handling the attributes and trajectory data. By referring to the results of HRNR-AT and those of GraphSAGE in {\LIANGMajor{Table \ref{tab:A_T_AT} and Table \ref{tab:classify}}}, HRNR-AT performs better than GraphSAGE, which is well aligned with the results in the original HRNR paper.}
% For example, the HRNR model used in our paper considers the default structure and spatial information as inputs, while HRNR-AT combines four types of information in the road network together. In the ``original HRNR paper'', the authors only consider the setting where all types of information are available, which is named HRNR-AT in our paper. As can be seen from Table \ref{tab:R11}, HRNR-AT significantly exceeds its counterpart GraphSAGE with huge improvement, which conforms to the conclusion obtained from the ``original HRNR paper''. Similar findings can also be witnessed from another application-specific baseline named Toast from Table \ref{tab:R11}.

% \begin{table}[h]
%     \renewcommand{\arraystretch}{1.05} 
% 	\centering
% 	\caption{Model performances for application-specific baselines.}
% 	\label{tab:R11}
% 	\resizebox{0.60 \linewidth}{!}{
% 		\begin{tabular}{@{}l|ccc|cc@{}}
% 			\toprule
%             \multirow{3}{*}{Default Setting} & \multicolumn{3}{c|}{{\it Road Type Classification}} & \multicolumn{2}{c}{{\it Travel Time Estimation}} \\
% 			\cmidrule{2-6}
% 			& Micro-F1 & Macro-F1 & Weighted-F1 & MAE & RMSE  \\ \midrule
% 		    GraphSAGE & 0.4955 & 0.3238 & 0.4648 & 151.83 & 219.88 \\ 
% 		    HRNR & 0.5050 & 0.2585 & 0.4399 & 168.35 & 244.09 \\
%             Toast & 0.4987 & 0.2697 & 0.4581 & 158.72 & 230.61 \\
% 			\bottomrule
% 			\toprule
% 			\multirow{3}{*}{+ Attributes} & \multicolumn{3}{c|}{{\it Road Type Classification}} & \multicolumn{2}{c}{{\it Travel Time Estimation}} \\
% 			\cmidrule{2-6}
% 			& Micro-F1 & Macro-F1 & Weighted-F1 & MAE & RMSE  \\ \midrule
% 		    HRNR-A & 0.6776 & 0.3670 & 0.6212 & 165.21 & 232.26 \\ 
% 		    Toast-A & 0.7353 & 0.4254 & 0.6792 & 155.06 & 208.78  \\
% 			\bottomrule
% 			\toprule
			
% 			\multirow{3}{*}{+ Trajectory} & \multicolumn{3}{c|}{{\it Road Type Classification}} & \multicolumn{2}{c}{{\it Travel Time Estimation}} \\
% 			\cmidrule{2-6}
% 			& Micro-F1 & Macro-F1 & Weighted-F1 & MAE & RMSE  \\ \midrule
% 		    HRNR-T & 0.5989 & 0.3244 & 0.5492 & 155.12 & 213.22 \\ 
% 		    Toast-T & 0.6210 & 0.3364 & 0.5695 & \underline{144.44} & \underline{205.18}  \\
% 			\bottomrule
% 			\toprule
			
% 			\multirowcell{3}{+ Attributes \& \\ Trajectory} & \multicolumn{3}{c|}{{\it Road Type Classification}} & \multicolumn{2}{c}{{\it Travel Time Estimation}} \\
% 			\cmidrule{2-6}
% 			& Micro-F1 & Macro-F1 & Weighted-F1 & MAE & RMSE  \\ \midrule
% 		    HRNR-AT & \underline{0.7060} & \underline{0.3823} & \underline{0.6473} & 154.98 & 208.87 \\ 
% 		    Toast-AT & \textbf{0.7512} & \textbf{0.4533} & \textbf{0.6996} & \textbf{142.23} & \textbf{199.52}  \\
% 			\bottomrule
% 	\end{tabular}}
% \vspace{-0.1cm}
% \end{table}

\vspace*{1\baselineskip}

\section*{Reviewer 2}

\centerline{\textbf{Comment D2.1}}
\noindent\emph{\textcolor{blue}{The hypergraph structure is constructed manually, instead of automatically learned. This restrict the applicability of this model.}}\\
\noindent\textbf{Response A2.1:} 
% Since we focus on road network, 
{\chengr We believe that} the intrinsic properties associated with the road network can be incorporated as prior knowledge. {\chengr Specifically, the way that} roads form local regions in the real world reflects rich semantic information. For example, those roads that constitute a highway loop (local region) would tend to have similar semantics. Therefore, we propose to build hypergraph structures {\chengr based on the regions' properties}.

% On the other hand, our construction strategy relies on a map segmentation algorithm which can be applied to any road network and obtain results automatically. From this point of view, our method is not that ``manually'' and can be widely applied to many scenarios.

\vspace*{1\baselineskip} 

\centerline{\textbf{Comment D2.2}}
\noindent\emph{\textcolor{blue}{When evaluating the models on travel time estimation, some of the works specifically designed for this task should be compared or discussed to show the advantage of the new proposed HGNN-based spatio-temporal analytical solution, e.g., [1, 2, 3].}}\\
\noindent\textbf{Response A2.2:} {\chengr We have included the following points for justifying our proposed model and experimental set-up of baseline methods.} \underline{First}, the methods proposed in these works are tailored for specific tasks such as traffic prediction, and the road representations learned for this specific task can hardly be transferred to other applications. In contrast, our method focuses on learning generic and transferable road representations which capture essential information of the road network and can be used to facilitate various downstream tasks.
%
\underline{Second}, these works often follow a supervised learning problem setting where large-scale labeled data is required. However, the large-scale labeled data could be expensive to obtain in some cases.
% and suffer from availability problems. 
In contrast, our method relies on unlabeled urban data such as road network structures as well as position information. It can be applied in different scenarios.
%
\underline{Third}, the objective of the experimental study in our paper is to evaluate the utility of the road network representations only. However, these specialized methods are highly dependent on the task-specific model designs and usually take more {\chengr data} as input and 
{\chengr it would not be fair to compare our model with these methods.}
% it is not a fair comparison any more. 
For example, [1] uses point of interest distributions as extra input; [2] {\chengr uses} weather and time interval as extra input; and [3] uses real-time traffic volume distributions as extra input. 
%
\underline{Fourth}, the experimental setup and baselines choice follow existing works \cite{wu2020learning, chen2021robust}. We have compared with \emph{all} methods that have been proposed for unsupervised road network representation learning as well as several representative graph representation learning methods (results are in Table \ref{tab:classify} and Table \ref{tab:tte} of this paper). 
% Therefore, this is a sufficiently comprehensive experimental comparison.

We have added some discussions on the provided references ([1], [2], [3]) in experimental setup (Section \ref{sec:R2_setting}, line 430-436).
\vspace*{1\baselineskip} 

\noindent{[1] Pan, Zheyi, et al. "Urban traffic prediction from spatio-temporal data using deep meta learning." Proceedings of the 25th ACM SIGKDD international conference on knowledge discovery \& data mining. 2019.}

\noindent{[2] Liang, Yuxuan, et al. "Urbanfm: Inferring fine-grained urban flows." Proceedings of the 25th ACM SIGKDD international conference on knowledge discovery \& data mining. 2019.}

\noindent{[3] Yao, Huaxiu, et al. "Revisiting spatial-temporal similarity: A deep learning framework for traffic prediction." Proceedings of the AAAI conference on artificial intelligence. Vol. 33. No. 01. 2019.}
\vspace*{1\baselineskip} 

\centerline{\textbf{Comment D2.3}}
\noindent\emph{\textcolor{blue}{Additionally, hypergraph neural networks have been applied to spatial-temporal mining and data prediction [4, 5]. It would be better to discuss the difference and novelty of the proposed Hypergraph Neural Network-enhanced spatio-temporal learning model.}}\\
\noindent\textbf{Response A2.3:} 
{\chengr Thank you for the comment. We discuss the difference between [4, 5] and our study in the following aspects.} \underline{First}, as for the modeling target, these methods mainly focus on region modeling. In contrast, our model is the first work to design hypergraph and hypergraph neural networks {\chengr for road network representation learning and more generally network network modelling}. 
%
\underline{Second}, as for the model design, these models employs HGNN only or stack GCN and HGNN hierarchically. {\chengr In contrast}, we {\chengr adopt a dual graph based approach} and aggregate information from both simple graph and hypergraph with separate channels. We are aware of no existing methods which use multiple channels to combine a simple graph and a hypergraph together as ours does.
%
\underline{Third}, as for the objective function design, these models apply commonly used supervised loss functions with the help of large-scale labeled data. In contrast, we propose a novel bi-level self supervised learning module, which involves not only the hypergraph reconstruction task, but also some other tasks such as hyperedge classification in the road network context ({\chengr which} is new). 

We have added {\chengr the above} comparisons {\chengr with} the provided references ([4], [5]) in introduction when discussing hypergraphs (Section \ref{sec:intro}, line 85-90).
\vspace*{1\baselineskip} 

\noindent{[4] Xia, Lianghao, et al. "Spatial-Temporal Sequential Hypergraph Network for Crime Prediction with Dynamic Multiplex Relation Learning." IJCAI. 2021.}

\noindent{[5] Luo, Xiaoyi, Jiaheng Peng, and Jun Liang. "Directed hypergraph attention network for traffic forecasting." IET Intelligent Transport Systems 16.1 (2022): 85-98.}
\vspace*{1\baselineskip} 
